Sparse Empirical Bayes Analysis (SEBA)

We consider a joint processing of $n$ independent sparse regression problems. Each is based on a sample $(y_{i1},x_{i1})...,(y_{im},x_{im})$ of $m$ \iid observations from $y_{i1}=x_{i1}\t\beta_i+\eps_{i1}$, $y_{i1}\in \R$, $x_{i 1}\in\R^p$, $i=1,...,n$, and $\eps_{i1}\dist N(0,\sig^2)$, say. $p$ is large enough so that the empirical risk minimizer is not consistent. We consider three possible extensions of the lasso estimator to deal with this problem, the lassoes, the group lasso and the RING lasso, each utilizing a different assumption how these problems are related. For each estimator we give a Bayesian interpretation, and we present both persistency analysis and non-asymptotic error bounds based on restricted eigenvalue - type assumptions.

==> SEBAproofsGroup.tex <==
\subsection{Proof of Section \ref{sec:grouped}}

\begin{proof}[Proof of Lemma \ref{lem:GroupLasso}]
a) Since \(\hat\beta\) minimizes \eqref{lassostar}, then,
\(\forall\beta\)
 \eqsplit{
    \sum_{ij} (Y_{ij}-x_{ij}\t\hat\beta_i)^2+\lm\sum_\ell
    \|\hat\beta_{\cdot\ell}\|_2
    &\leq
    \sum_{ij} (Y_{ij}-x_{ij}\t\beta_i)^2+\lm\sum_\ell
    \|\beta_{\cdot\ell}\|_2
  }
Then for \(f_{ij}=Y_{ij}-\eps_{ij}\), \(\eps_{ij}\dist\normal(0,\sig^2)\)
\iid, since
 \eqsplit{
    \|f-\hat f\|_2^2 &= \sum_{ij}(Y_{ij}-x_{ij}\t\beta_i-\eps_{ij})^2
    \\
    &= \sum_{ij} (Y_{ij}-x_{ij}\t\beta_i)^2 + \sum_{ij} \eps_{ij}^2 +
    2\sum_{ij}\eps_{ij}(x_{ij}\t\beta_i-Y_{ij}),
  }
we have
 \eqsplit{
    \|f-\hat f\|_2^2 + \lm\sum_\ell \|\hat\beta_{\cdot\ell}\|_2
    &\leq \|f_{\beta}-f\|_2^2 + \lm\sum_{\ell}\|\beta_{\cdot\ell}\|_2
    +2\sum_{ij}\eps_{ij}x_{ij}\t(\beta_i-\hat\beta_i)
  }
The last term can be bounded with high probability. Denote
\(V_{il}=\summ j1m x_{ij\ell}\eps_{ij}\dist\normal(0,\sig^2\sum_j
x_{ij\ell}^2)\). Denote the event \(\sca_\ell=\bigcap_{i=1}^n
\{|V_{i\ell}|\leq c_{il}\}\), for some \(c_{i\ell}>0\). Then
 \eqsplit{
    P(\sca_\ell^c) &\leq \summ i1n P(|V_{i\ell}|>c_{i\ell})
    \\
    &= \summ i1n 2\biggl[1-\Phi\Bigl\{c_{i\ell}/\sig\bigl(\sum_j
    x_{ij\ell}^2\bigr)^{1/2}\Bigr\}\biggr]
    \\
    &\leq \summ i1n \exp\bigl\{- c_{i\ell}^2/2\sig^2\sum_jx_{ij\ell}^2\bigr\}
    \\
    &= n\exp\bigl\{-\mu^2/2\sig^2\bigr\}
  }
where \(c_{il}\equiv \mu^2 \sum_j x_{ij\ell}^2\).

Now, for the event \(\sca=\bigcup_{\ell=1}^p
\sca_{\ell}=\bigcup_\ell\bigcup_i\{|V_{i\ell}|\le c_{i\ell}\}\),
 \eqsplit{
    P(\sca^c) &\leq \summ \ell 1p P(\sca_\ell^c) \leq npe^{-\mu^2/2\sig^2}.
  }%
Thus, if \(\mu\) is large enough \(P(\sca^c)\) is small. E.g., for \(\mu=\sig A\bigl(\log(np)\bigr)^{1/2}\),
\(A>\sqrt 2\), we have \(P(\sca^c)\leq (np)^{1-A^2/2}\).

Back to the bound for \(\|f-\hat f\|+\lm
\sum_\ell\|\hat\beta_{\cdot\ell}\|^2\). We have that on \(\sca\),
 \eqsplit{
    \|f-\hat f\|_2^2 &\leq \|f_\beta -f\|_2^2 + \lm\sum_\ell
    \bigl(\|\beta_{\cdot\ell}\|_2 - \|\hat\beta_{\cdot\ell}\|_2\bigr)
    +2\sum_{i\ell}c_{il}|\beta_{il}-\hat\beta_{i\ell}|\\
   &\leq \|f_\beta -f\|_2^2 + \lm\sum_\ell
    \bigl(\|\beta_{\cdot\ell}\|_2 - \|\hat\beta_{\cdot\ell}\|_2\bigr)
    +2\sum_{\ell} \sqrt{\sum_i c_{il}^2 }| ||\beta_{\cdot \, l}-\hat\beta_{\cdot \,
    \ell}||_2,
    }
since \(V_{i\ell}(\beta_{i\ell}-\hat\beta_{i\ell})\leq
c_{i\ell}|\beta_{i\ell}-\hat\beta_{i\ell}|\) on \(\sca\).

Let \(\ti\lm>0\). Add now
\(\ti\lm\sum_{\ell}\|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2\) to both
sides
 \eqsplit{
    \|f-\hat f\|_2^2 + \ti\lm \sum_\ell \|\beta_{\cdot\ell}
    -\hat\beta_{\cdot\ell}\|_2
    &\leq \|f_\scb - f\|_2^2
    + \ti\lm \sum_\ell \|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2
    +\lm\sum_\ell \|\beta_{\cdot\ell}\|_2
    \\
    &\hspace{2em}
    -\lm\sum_\ell \|\hat\beta_{\cdot\ell}\|_2
    +2\max_{\ell} \sqrt{\sum_i c_{il}^2 } \,\, \sum_{\ell}||\beta_{\cdot \, l}-\hat\beta_{\cdot \,
    \ell}||_2,
    \\
    &= \|f_\beta - f\|_2^2
    +\sum_\ell S_{\beta\ell},\qquad\text{say.}
  }

Now, for \(\ell\not\in J(\beta)\),
 \eqsplit{
    S_{\beta\ell} &= \ti\lm \|\hat\beta_{\cdot\ell} \|_2 -\lm
    \|\hat\beta_{\cdot\ell}\|_2 +
2 ||\hat\beta_{\cdot \, \ell}||_2 \,  \max_{\ell} \sqrt{\sum_i
c_{il}^2 }
     \\
    &= \|\hat\beta_{\cdot\ell}\|_2 \Bigl(\ti\lm-\lm
    + 2\max_{\ell} \sqrt{\sum_i c_{il}^2 } \Bigr)
  }
This expression can be negative if \(\lm>2\max_{\ell} \sqrt{\sum_i
c_{il}^2 }  \) and \(0\leq\ti\lm \leq \lm - 2\max_{\ell}
\sqrt{\sum_i c_{il}^2 } \).


On the other hand, for \(\ell\in J(\beta)\):
 \eqsplit{
    S_{\beta\ell} &\leq  \|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2 \left( \ti \lm+\lm + 2 \max_{\ell} \sqrt{\sum_i c_{il}^2 } \right)
  }
Thus,
 \eqsplit{
    \|\hat f- f\|_2^2 +\ti\lm \sum_\ell
    \|\hat\beta_{\cdot\ell}-\beta_{\cdot\ell}\|_2
    &\leq \|f_\beta - f\|_2^2 + \left(\lm + \ti\lm + 2\max_{\ell} \sqrt{\sum_i c_{il}^2 }\right) \, \sum_{\ell\in J(\beta)} \|\hat \beta_{\cdot\ell}
    -\beta_{\cdot\ell}\|_2.
  }

We have, therefore, the following conditions on \(\mu\) and \(\ti\lm\):
 \eqsplit[nb1]{
    \ti\lm &\leq \lm - 2\mu  \max_{\ell} \sqrt{\sum_{i,j}
    x_{ij\ell}^2}\;\;,\qquad\ell=1,\dots,p.
    \\
    \implies \lm &> 2\mu \max_{\ell} \sqrt{\sum_{i,j}
    x_{ij\ell}^2}\;\;,\qquad\ell=1,\dots,p.
  }
  Recall that $\mu = A\sig\sqrt{\log(np)}, \quad A>\sqrt 2$.
Thus, for example one can take
 \eqsplit{
    \ti\lm &= \lm/2 = 2 \mu\max_{\ell} \sqrt{\sum_{i,j} x_{ij\ell}^2}
} which implies that
 \eqsplit{
    \mu&= \frac{\lm} {4\Lm_x},%\quad \Lm_x=A\sig\sqrt{\log(np)}
    \\
    \Lm_x&= \max_{\ell}\sqrt{\sum_{ij} x_{ij\ell}^2}
    \\
    \text{i.e.,  } \lm &= 4 \mu \Lm_x = 4 A\sig \Lm_x \sqrt{\log(np) }.
  }
Then,
 \eqsplit{
    \lm^2-\mu^2\max_\ell \sum_{i,j} x_{ij\ell}^2
    =\frac{15}{16}\lm^2,
  }
which concludes the proof of part (a).

b) Similarly, for the $\ell_1$ norm of the difference between the
betas we have, for some $\lm_1 >0$:
 \eqsplit{
    \|f-\hat f\|_2^2 +  \lm_1 \sum_\ell \|\beta_{\cdot\ell}
    -\hat\beta_{\cdot\ell}\|_1
    &\leq \|f_\scb - f\|_2^2
    +  \lm_1 \sum_\ell
    \|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_1
    +\lm\sum_\ell \|\beta_{\cdot\ell}\|_2
    \\
    &\hspace{2em}
    -\lm\sum_\ell \|\hat\beta_{\cdot\ell}\|_2
    + 2\sum_\ell \max_i c_{i\ell}\|\beta_{\cdot\ell} -
    \hat\beta_{\cdot\ell}\|_1
    \\
    &= \|f_\beta - f\|_2^2
    +\sum_\ell \ti S_{\beta\ell},\qquad\text{say.}
  }

For \(\ell\not\in J(\beta)\),
 \eqsplit{
    \ti S_{\beta\ell} &\leqslant  \lm_1 \|\hat\beta_{\cdot\ell} \|_1 -\lm
    \|\hat\beta_{\cdot\ell}\|_2 + 2\sqrt{\sum_i
    c_{i\ell}^2 } \|\hat\beta_{\cdot\ell}\|_2
    \\
    &\leq   \|\hat\beta_{\cdot\ell}\|_2 \Bigl( \lm_1 \sqrt{n} -\lm
    +\sqrt{\sum_i     c_{i\ell}^2 } \Bigr)
  } % n can be replaced with \scm(\hat\beta_{\cdot\ell})

This expression is negative if \(\lm>2\sqrt{\sum_i
    c_{i\ell}^2 } + \lm_1 \sqrt{n} >0 \).

On the other hand, for \(\ell\in J(\beta)\):
 \eqsplit{
    \ti S_{\beta\ell} &\leq \left( \lm_1 + \lm + 2\sqrt{\sum_i
    c_{i\ell}^2 }\right) \|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2
  }
Thus, similarly to part a), we can take $\lm_1 \sqrt{n} = \ti\lm =
2 \mu\max_{\ell}\sqrt{\sum_{ij} x_{ij\ell}^2} = \lambda/2$ and the
same $\mu$ and $\lm$ as in a).

c) We have
 \eqsplit{
    \sum_j x_{ij\ell}(Y_{ij} -x_{ij}\t\hat\beta_i) &=\lm
    \frac{\hat\beta_{i\ell}} {\Bigl(\sum_k
    \hat\beta_{k\ell}^2\Bigr)^{1/2}}\, ,
  }
and on \sca,
 \eqsplit{
    \Bigl|\sum_j x_{ij\ell}(Y_{ij}-f_{ij})\Bigr| \leq c_{i\ell}=\mu \Bigl(\sum_j
    x_{ij\ell}^2\Bigl)^{1/2}.
  }
Thus, on \(\sca\),
 \eqsplit{
    \sum_{ij}\bigl(x_{ij\ell}(f_{ij} - x_{ij}\t\hat\beta_i)\bigr)^2
    &\geq \frac1m \sum_i\Bigl(\sum_j x_{ij\ell}(f_{ij}
    -x_{ij}\t\hat\beta_i)\Bigr)^2
    \\
    &\geq \frac1m \sum_i \Bigl(\sum_j
    x_{ij\ell}(Y_{ij}-x_{ij}\t\hat\beta_i)\Bigr)^2
    -\frac1m \sum_i \Bigl(\sum_j x_{ij\ell}(f_{ij}-Y_{ij})\Bigr)^2
    \\
    &\geq \frac1m \sum_i\lm^2 \frac{\beta_{i\ell}^2} {\sum_i\beta_{i\ell}^2}
    -\frac1m \sum_{i:\hat\beta_{i\ell}\ne 0}c_{i\ell}^2
    \\
    &= \frac1m\Bigl(\lm^2-\mu^2\sum_{i:\hat\beta_{i\ell}\ne 0}
    x_{ij\ell}^2\Bigr).
  }

%Now, the pattern of \(\hat\beta_{i\ell}\) is the same for fixed
%\(\ell\), i.e., if \(\hat\beta_{1\ell}=0\) then
%\(\hat\beta_{i\ell}=0\), \(i=1,\dots,n\) (or it is so with
%probability 1???????)[NB: this is true if $X_i = X$ ie is
%independent of $i$, otherwise t does not follow?].
Therefore
 \eqsplit{
    \sum_{i,j,\ell}\Bigl(x_{ij\ell}(f_{ij} -
    x_{ij}\t\hat\beta_i)\Bigr)^2
    &\geq \frac1m
    \sum_{\ell:\hat\beta_{i\ell}\ne0}\Bigl(\lm^2 - \mu^2\sum_{ij}x_{ij\ell}^2\Bigr)
    \\
    &\geq \scm(\hat\beta)\frac1m\Bigl(\lm^2-\mu^2\max_{\ell}\sum_{ij}x_{ij\ell}^2\Bigr)
    \\
    &= \scm(\hat\beta)\frac1m \Bigl(\lm^2 - \mu^2\max_{\ell}\sum_{ij}x_{ij\ell}^2\Bigr)
    \\
    &= \scm(\hat\beta) \frac1m \Bigl(\lm^2-\mu^2 \max_{\ell}\sum_{ij}x_{ij\ell}^2\Bigr)
  }
On the other hand,
 \eqsplit{
    \sum_{ij\ell}\Bigl(x_{ij\ell}(f_{ij} -
    x_{ij}\t\hat\beta_i)\Bigr)^2
    &\leq \sum_\ell \max_{ij}
    x_{ij\ell}^2\|f-\hat f\|^2
  }
thus implying that
 \eqsplit{
    \scm(\hat\beta) &\leq \|f - \hat f\|_2^2
    \frac{\sum_\ell\max_{i,j}x_{ij\ell}^2} {\lm^2-\mu^2\max_\ell
    \sum_{i,j}x_{ij\ell}^2}.
  }
Lemma is proved.
\end{proof}





\begin{proof}[Proof of Theorem \ref{th:BRT61}]
Fix an arbitrary $\beta\in\mathbb{R}^p$ such that $\scm(\beta)\le
s$.
 On event $\sca$ defined in the proof of Lemma 1, inequalities
\eqref{boundf} hold. Consider two cases.

\begin{enumerate}
\item $  2\lambda \sum_{\ell \in J(\beta)} ||\beta_{\cdot\ell} -
\hat\beta_{\cdot\ell}||_1  \leqslant \varepsilon || f -
f_{\scb}||_2^2$. In this case, the result of the theorem follows
trivially from \eqref{boundf}.

\item $\varepsilon || f - f_{\scb}||_2^2 < 2\lambda \sum_{\ell \in
J(\beta)} ||\beta_{\cdot\ell} - \hat\beta_{\cdot\ell}||_1 $.
Denote the event  defined by this  inequality by $\tilde\sca$; all
subsequent inequalities hold on $\sca \cap \tilde\sca$.


On this event, we get from \eqref{boundf} that
$$
\sum_{\ell \in J^c(\beta)}  ||\beta_{\cdot\ell} -
\hat\beta_{\cdot\ell}||_1 \leqslant  4\sqrt{n} (1+1/\varepsilon)
\sum_{\ell \in J(\beta)} ||\beta_{\cdot\ell} -
\hat\beta_{\cdot\ell}||_1.
$$
Assumption URE$_n(s, 4\sqrt{n} (1+1/\varepsilon))$ implies that
$$
\kappa^2 \sum_{\ell \in J(\beta)} |\beta_{i\ell} -
\hat\beta_{i\ell}|_2^2 \leqslant || X_{i\cdot\cdot}\t
(\beta_{i\cdot } - \hat\beta_{i\cdot }) ||_2^2 = || f_{\rb \,
i\cdot } - \hat{f}_{i\cdot } ||_2^2,
$$
where $\kappa = \kappa(s, 4\sqrt{n} (1+1/\varepsilon))$. (For
other assumptions, use the corresponding $\kappa$; for MRE2 use a)
of Lemma~\ref{lem:GroupLasso}).

 Hence,
by \eqref{boundf},
\begin{eqnarray*} %check
 \|f-\hat f\|_2^2  &\le&  \|f - f_{\scb}\|_2^2
     +2\lm \sum_{\ell\in J(\beta)}\|\hat\beta_{\cdot\ell}
     -\beta_{\cdot\ell}\|_2\\
     &\le&  \|f - f_{\scb}\|_2^2 +
     2\lm \sqrt{\scm(\beta)} \left[\sum_{\ell\in J(\beta)}\|\hat\beta_{\cdot\ell}
     -\beta_{\cdot\ell}\|_2^2\right]^{1/2}\\
     &=&  \|f - f_{\scb}\|_2^2 +
     2\lm \sqrt{\scm(\beta)} \left[\sum_{i=1}^n\sum_{\ell\in J(\beta)} |\hat\beta_{i \ell}
     -\beta_{i \ell}|_2^2\right]^{1/2}\\
     &\le&  \|f - f_{\scb}\|_2^2 +
     2\lm \sqrt{\scm(\beta)} \left[\sum_{i=1}^n  \frac 1 {\kappa^2} \|\hat{f}_{i\cdot} - f_{\scb\, i\cdot}\|_2^2
     \right]^{1/2}\\
     &=&  \|f - f_{\scb}\|_2^2 +
     2\lm \frac{\sqrt{\scm(\beta)}}{\kappa}   \|\hat{f}  - f_{\scb }\|_2\\
     &\le&  \|f - f_{\scb}\|_2^2 +
     2\lm \frac{\sqrt{\scm(\beta)}}{\kappa} \left[  \|\hat{f}  - f \|_2 + \|f  - f_{\scb }\|_2 \right].
\end{eqnarray*}
Using inequality $2xy \le  x^2/b +   b y^2$ with $b\in(0,1)$, $x =
\lm \sqrt{\scm(\beta)}/\kappa$, and $y$ being either $\|\hat{f}  -
f \|_2$ or $\|f  - f_{\scb }\|_2$, we can decouple the last term
to obtain
\begin{eqnarray*}
 \|f-\hat f\|_2^2 &\le& \frac{1+b}{1-b} \|f - f_{\scb}\|_2^2 +
      \frac{2 \lm^2\scm(\beta)}{b(1-b)\kappa^2}, \quad \forall b\in(0,1).
\end{eqnarray*}
Taking $b=\left(1+2/\varepsilon\right)^{-1}$ we obtain
\begin{eqnarray*}
 \|f-\hat f\|_2^2 &\le& (1+\varepsilon) \|f - f_{\scb}\|_2^2 +
      \frac{\lm^2\scm(\beta) (\varepsilon+2)^2}{\varepsilon
      \kappa^2}.
\end{eqnarray*}
 Substituting the value of $\lm$ and taking the infimum over all considered $\beta$ finishes the proof of the theorem.
\end{enumerate}

\end{proof}


==> SEBAproofsRINGS.tex <==
\begin{comment}

\begin{proof}[Proof] of Theorem~\ref{th:persistRINGS}.

Similarly to the proof of Theorem~\ref{th:lassoes1}, we can show
that \eqsplit{ mnL_F(\scb_F^*) + \lm |||\hat\scb|||_1^{\alpha}
\leqslant mn L_F(\scb ) + \lm |||\scb|||_1^{\alpha} + m\delta_n
\summ i1n \left(\|\beta_i\|_1^2 + \|\hat\beta_i\|_1^2 \right). }

Since \eqsplit { \summ i1n ||\beta_i||_1^2 \leqslant p
||\scb||_2^2 = p |||\scb|||_2^2 \leqslant p |||\scb|||_1^2, }
 we have
 \eqsplit[eq:persist-RINGalpha]{ mn L_F(\scb_F^*) + \lm |||\hat\scb|||_1^{\alpha}
\leqslant mn L_F(\scb ) + \lm |||\scb|||_1^{\alpha} + p m \delta_n
\left( |||\scb|||_1^2 +  |||\hat\scb|||_1^2 \right), } i.e. that
 \eqsplit{  \lm |||\hat\scb|||_1^{\alpha} - p m
\delta_n |||\hat\scb|||_1^2 \leqslant mn (L_F(\scb)-
L_F(\scb_F^*)) + \lm |||\scb|||_1^{\alpha} + p m \delta_n
|||\scb|||_1^2. }


We consider this for $\alpha=1$, $\alpha=2$ and for $\alpha >2$
separately.

Denote $w = \frac{\lm}{mp\delta}$, $d= \frac{n}{p\delta}
(L_F(\scb)- L_F(\scb_F^*)) + w |||\scb|||_1^{\alpha} +
|||\scb|||_1^2$. For $\alpha =1$, we have a quadratic inequality
for $z = |||\hat\scb|||_1$: $ z^2 - w z + d \geqslant 0$, with
solutions  $z\leqslant \frac 1 2 (w - \sqrt{w^2-4d})$ and
$z\geqslant \frac 1 2 (w + \sqrt{w^2-4d})$, if $w> 2\sqrt{d}$. If
$w \leqslant 2\sqrt{d}$, the inequality is satisfied for all $z$.
Hence, for $\alpha =1$, the method does not give an upper bound
for $|||\beta|||_1$.

For $\alpha = 2$, if $\lm \leqslant pm\delta_n$, we cannot derive
an upper bound on $|||\hat\scb|||_1$. If $\lm > pm\delta_n$,
\eqsplit{ |||\hat\scb|||_1 \leqslant \frac{\lm n}{p\delta}
(L_F(\scb)- L_F(\scb_F^*)) + \frac{\lm + pn\delta}{\lm - pn\delta}
||| \scb|||_1. }

For $\alpha > 2$: assume that $\lm \leqslant pm\delta_n$. Then,
similarly to the proof of Theorem~\ref{th:lassoes2}, we have that
$|||\hat\scb|||_1$ is maximised subject to constraint
\eqref{eq:persist-RINGalpha} when it solves equation $\lm u^\al
-pm\delta_n u^2 = \O(pm\delta_n)$, implying that $u=\O\left(
\left(\frac{\lm}{mp\delta_n}\right)^{1/(\al-2)} \right)$, i.e.
\eqsplit{ |||\hat\scb|||_1 \leqslant  \O\left(
\left(\frac{\lm}{mp\delta_n}\right)^{1/(\al-2)} \right). }


Also, we have, similarly to  \eqref{bpl1},
 \eqsplit{
    \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    &\leq   \summ i1n \ti\beta_{i}\t\ti S_i \ti\beta_{i}
    + \frac{\lm_n}m   ||| \scb|||_1^\al
    -  \frac{\lm_n}m  |||\hat\scb|||_1^\al
    +  \del_n\summ i1n \|\tihat\beta_{i}\|_1^2
    \\
    &\leq   \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    + \frac{\lm_n}m |||\scb|||_1^\al
    -  \frac{\lm_n}m  |||\hat\scb|||_1^\al
    +  \del_n \summ i1n \| \beta_{i}\|_1^2
    + \del_n \summ i1n \|\hat\beta_i\|_1^2 +2n\delta_n
    \\
    &\leq   \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    + \frac{\lm_n}m ||| \scb|||_1^\al
    -  \frac{\lm_n}m  |||\hat\scb|||_1^\al
    + p \del_n \left( |||\scb|||_1^2 +  |||\hat\scb|||_1^2
    \right)  +2n\del_n.
  }

Hence, for $\alpha = 2$ and $\lm > pm\delta_n$,

\eqsplit{
    \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    &\leq   \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    + 2(\frac{\lm_n}m +p\del_n) ||| \scb|||_1^2
    + \lm n(1-  \frac{\lm_n}{m p \del_n}) \left(  L_F(\scb)-
L_F(\scb_F^*) \right)
         +2n\del_n.
 }

For $\alpha > 2$ and $\lm < pm\delta_n$, \eqsplit{
    \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    &\leq   \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    + \frac{\lm_n}m ||| \scb|||_1^\al + p \del_n |||\scb|||_1^2
    -  \frac{\lm_n}m  \O\left(
\left(\frac{\lm}{mp\delta_n}\right)^{\al/(\al-2)} \right)\\
    &+ p \del_n \O\left(
\left(\frac{\lm}{mp\delta_n}\right)^{2/(\al-2)} \right)
       +2n\del_n.
}

Assuming that $\lm \ll pm\delta_n$, we have \eqsplit{
    \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    &\leq   \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    +   \O((p+n) \del_n)\\
    &+ p \del_n  \O\left(
\left(\frac{\lm}{mp\delta_n}\right)^{2/(\al-2)} \right) \left[ 1 -
  \frac{\lm_n}{mp\del_n}  \O\left(
\left(\frac{\lm}{mp\delta_n}\right) \right) \right]\\
    &=   \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    +   \O((p+n) \del_n)+ p \del_n \O\left(
\left(\frac{\lm}{mp\delta_n}\right)^{2/(\al-2)} \right).
  }

\end{proof}
\end{comment}

==> SEBAproofsSpectralTMP.tex <==
\subsection{Proofs of Section \ref{sec:spectral} }

\begin{proof}[Proof of Lemma \ref{lem:psiConvex}]
Let \(A(t) = \sum \bigl(\beta_i(t)+ t\ti\beta_i(t)\bigr)\bigl(\beta_i(t)+ t\ti\beta_i(t)\bigr)\t = \sum \beta_i\beta_i\t + t(\sum \beta_i\ti\beta_i\t + \sum \ti\beta_i\beta_i\t) + t^2\sum\ti\beta_i\ti\beta_i\t\).  Let \(x_1(t),\dots,x_p(t)\) be a smooth orthonormal basis of eigenvectors of $A(t)$, and \(A(t) = \sum c_i(t)x_i(t)x_i(t)\t\).


Denote by $\dot{}$ and $\ddot{}$ the first and second derivative, respectively, according to $t$. Then, note that taking the derivative of \(x_i\t x_i=1\) yields \(x_i\t\dot x_i=0\), and trivially, since $x_i$ is an eigenvector,  also \(x_i\t A\dot x_i=0\). Differentiating \(A(t)x_k(t) = c_k(t) x_k(t) \):
 \eqsplit{
    \dot A x_k + A\dot x_k &= \dot c_k x_k + c_k\dot x_k.
  }
But $\dot x_k\perp x_k$, hence
 \eqsplit{
    \dot x_i &= -(A - c_k I)^+\dot A x_k
  }
Hence, generally:
 \eqsplit[eigender]{
    c_k &= x_k\t A x_k
    \\
    \dot c_k &= x_k\t \dot A x_k  \qquad\qquad\qquad\text{(Recall \(\dot x_k\perp x_k\))}
    \\
    \ddot c_k &= 2 x_k\t \dot A \dot x_k + x_k \t\ddot A x_k.
    \\
    &= -2x_k\t\dot A (A-c_kI)^+\dot Ax_k +   x_k \t\ddot A x_k.
  }
For the particular matrices \(A(t)\):
 \eqsplit{
    c_k &= \sum (x_k\t\beta_i)^2
    \\
    \dot c_k &= 2\sum (x_k\t\beta_i) (x_i\t \ti \beta_k)
    \\
    \ddot c_k &=  -2 x_k\t \bigl(\sum \beta_i\ti\beta_i\t + \sum \ti\beta_i\beta_i\t\bigr) \bigr(\sum_{i\ne k} \frac1{c_i-c_k}x_ix_i\t\bigl)\bigl(\sum \beta_i\ti\beta_i\t +\sum \ti\beta_i\beta_i\t\bigr)x_k
     \\
     &\hspace{3em}+ 2\sum_i (x_k\t\ti\beta_i)^2
    \\
    &= -2 \sum_i \sum_{j\ne k} \sum_m \frac1{c_j-c_k} (x_k\t\beta_i)(x_j\t\ti\beta_i)(x_j\t\ti\beta_m)
    (x_k\t\beta_m)
    \\
    & \hspace{3em }-4\sum_i \sum_{j\ne k} \sum_m \frac1{c_j-c_k} (x_k\t\beta_i)(x_j\t\ti\beta_i)(x_j\t\beta_m)(x_k\t\ti\beta_m)
    \\
    & \hspace{3em }- 2 \sum_i \sum_{j\ne k} \sum_m \frac1{c_j-c_k} (x_k\t\ti\beta_i)(x_j\t\beta_i)(x_j\t\beta_m)
    (x_k\t\ti\beta_m)
    \\
     &\hspace{3em}+ 2\sum_i (x_k\t\ti\beta_i)^2
    \\
    &= -2\sum_{j\ne k} \frac1{c_j-c_m}\Bigl(\sum_i (x_k\t\beta_i)(x_j\t\ti\beta_i) + \sum_i (x_k\t\ti\beta_i)(x_j\t\beta_i)\Bigr)^2
    \\
     &\hspace{3em}+ 2\sum_i (x_k\t\ti\beta_i)^2
  }
Now,
 \eqsplit{
    \frac{d^2}{dt^2}\sqrt{c_k(t)}\Bigl|_{t=0}&=\frac{d}{dt}\frac{\dot c_k}{2c_k^{1/2}} = \frac{2\ddot c_k c_k - \dot c_k^2 }{4c_k^{3/2}}
  }
Hence
 \eqsplit{
    \sum_k \frac{d^2}{dt^2}\sqrt{c_k(t)}\Bigl|_{t=0}
    &= 2\sum_k \frac{\sum_i (x_k\t\ti\beta_i)^2\sum_i (x_k\t\beta_i)^2 - \bigl(\sum_i (x_k\t\beta_i)(x_k\t\ti\beta_i)\bigr)^2}{4c_k^{3/2}}
    \\
    &\hspace{3em} -\sum_k\sum_{j\ne k} \frac1{c_j-c_k}\frac{\Bigl(\sum_i (x_k\t\beta_i)(x_j\t\ti\beta_i) + \sum_i (x_k\t\ti\beta_i)(x_j\t\beta_i)\Bigr)^2}{c_k^{1/2}}
    \\
    &=  2\sum_k \frac{\sum_i (x_k\t\ti\beta_i)^2\sum_i (x_k\t\beta_i)^2 - \bigl(\sum_i (x_k\t\beta_i)(x_k\t\ti\beta_i)\bigr)^2}{4c_k^{3/2}}
    \\
    &\hspace{3em} +2\sum_k\sum_{j> k} \frac{\Bigl(\sum_i (x_k\t\beta_i)(x_j\t\ti\beta_i) + \sum_i (x_k\t\ti\beta_i)(x_j\t\beta_i)\Bigr)^2}{c_k^{1/2}c_j^{1/2} (c_k^{1/2}+c_j^{1/2})}
    \\
    &\ge 0.
  }
Since \(\psi(\beta_1+t\ti\beta_1,\dots,\beta_p+t\ti\beta_p) = \sum_k\sqrt{c_k(t)}\), the lemma was proven.
\end{proof}



\begin{proof}[Proof of Theorem \ref{th:sparseSpect}]

Since the target function is invariant to rotation of $x$ and $\beta$ at the same time, we assume for simplicity that $U=I$. Suppose that \(S\) is the set of non-zero components of the estimator. Let $\hat\beta_{S}\in\R^{|S|+`}$ be the vector of nonzero entries of $\hat\beta$ in the first $|S|$ places and 0 in the $(|S|+1)$ place, let $X_{Si}$ be the corresponding columns extracted from the covariates matrix $X_i$ of the $i$-th trial. Let \(\beta_{iN}\) be \(b_i e_{|S|+1}\), where \(\ell\not\in S\), and \(e_\ell\) is the standard vector with 1 at the \(\ell\)-th position and 0 otherwise. Consider now the target function at a small neighborhood \(t=0\):
 \eqsplit{
    \sum_i \sum_j \|y_{ij} -x_{Sij}\t\hat\beta_{Si}+tx_{ij\ell}b_i)\|^2 + \lm\psi (\beta_{1S}+t\beta_{1N},\dots,\beta_{nS}+t \beta_{nN}).
  }
Now the spectrum is not changed by elementary operations. Hence
 \eqsplit{
    &\hspace{-3em}\spect\begin{pmatrix} \sum \hat\beta_i\hat\beta_i\t & t\sum b_i\hat\beta_i \\ t\sum b_i \hat\beta_i\t & t^2\sum b_i^2 \end{pmatrix}
    \\
    &= \spect\begin{pmatrix} \sum_i \hat\beta_i\hat\beta_i\t &  0 \\ 0 & t^2\sum b_i^2 - t^2\sum_i b_i\hat\beta_i\t \Bigl(\sum_i \hat\beta_i\hat\beta_i\t\Bigr)^{-1} \sum_ib_i\hat\beta_i \end{pmatrix}
    \\
    &= \spect\Bigl(\sum \hat\beta_i\hat\beta_i\t\Bigr) \union t^2 \bigl(\sum b_i^2 - \sum_i b_i\hat\beta_i\t \Bigl(\sum_i \hat\beta_i\hat\beta_i\t\Bigr)^{-1} \sum_ib_i\hat\beta_i \bigr),
  }
where $\spect A$ is the spectrum of the matrix $A$. Hence
 \eqsplit{
    &\hspace{-3em}\frac{\partial}{\partial t}\psi (\beta_{1S}+t\beta_{1N},\dots,\beta_{nS}+t \beta_{nN})
    \\
    &=\sgn(t)
    \bigl(\sum b_i^2 - \sum_i b_i\hat\beta_i\t \Bigl(\sum_i \hat\beta_i\hat\beta_i\t\Bigr)^{-1} \sum_ib_i\hat\beta_i \bigr)^{1/2}
  }
Which means that the optimal \(t\) will be zero if for all i
 \eqsplit{
    |\sum_j x_{ij\ell}(y_{ij} - x_{Sij}\t \beta_{Si})| & \leq \lambda\bigl(1 - \hat\beta_i\t \Bigl(\sum_k \hat\beta_k\hat\beta_k\t\Bigr)^{-1} \hat\beta_i \bigr)^{1/2}
  }

\end{proof}


==> SEBAsecLassoes-1.tex <==
\section{The lassoes procedure }
\label{sec:lassoes}

\subsection{Definition and persistence}

The  minimal structural relationship we may assume is that the
$\beta's$ are not related, except that we believe that there is a
bound on the average sparsity of the $\beta$'s. One possible
approach would be to consider the problem as a standard sparse
regression problem with $nm$ observations, a single vector of
coefficients $\beta=(\beta_1\t,\dots,\beta_n\t)\t$, and a block
diagonal design matrix $X$. This solution imposes very little on
the similarity among $\beta_1,\dots,\beta_n$.


We assume that each
vector $\beta_i$ solves a different problem, and these problems
are related only through the joint loss function, which is the sum
of the individual losses. To be clearer, we assume that for each
$i=1,\dots,n$,   $z_{ij}=(y_{ij}, x_{ij}\t)\t$, $j=1,\dots,m$ are
\iid, sub-Gaussian random variables, drawn from a distribution
$Q_i$. Let $z_i=(y_i,x_i\t)\t$ be an independent sample from
$Q_i$. For any vector $a$, let  $\ti a=(-1,a\t)\t$, and let
$\tilde\Sig_i$ be the covariance matrix of $z_i$ and
$\mathfrak{S}=(\ti\Sig_1,\dots,\ti\Sig_n)$. The goal is to find
the matrix $\hat\scb=(\hat\beta_1,\dots,\hat\beta_n)$ that
minimizes the mean prediction error:
 \eqsplit[persis]{
    L(\scb,\mathfrak S) &= \summ i1n \E_{Q_i}(y-x_i\t\beta_i)^2=\summ i1n \ti\beta\t\ti\Sig_i\ti\beta.
  }
For $p$  small, the natural approach is empirical risk
minimization, that is replacing $\ti\Sig_i$ in \eqref{persis} by
$\ti S_i$, the empirical covariance matrix of $z_i$. However,
generally speaking, if $p$ is large, empirical risk minimization
results in  overfitting the data. Greenshtein and Ritov
\cite{p:GR-persist} suggested minimization over a restricted set
of possible $\beta$'s, in particular, to either  $L_1$ or $L_0$
balls. In fact, their argument is based on the following
simple observation
 \eqsplit[roughapprox]{
    \bigl| \ti\beta\t(\ti\Sig_i - \ti S_i)\ti\beta\bigr|
    &\leq \| \ti\Sig_i - \ti S_i \|_\en \|\ti\beta\|_1^2
    \\
    &\hspace{-10em}\text{and}
    \\
    \| \ti\Sig_i - \ti S_i \|_\en &=\O_p(m^{-1/2}\log p)
  }
%NB 19 Nov
(see Lemma~\ref{lem:persist} in the Appendix.)

This leads to  the natural extension of the single vector lasso to
the compound decision problem set up, where we penalize by the sum
of the \emph{squared} $L_1$ norms of vectors
$\ti\beta_1,\dots,\ti\beta_n$, and obtain the estimator defined
by:
 \eqsplit[lassoes]{
    (\dacc\ti\hat\beta_i,\dots,\dacc\ti\hat\beta_n)
    &=\argmin_{\ti\beta_1,\dots,\ti\beta_n} \Bigl\{m\summ i1n \ti\beta_i\t\ti S_i\ti\beta_i
    + \lm_n \summ i1n \|\ti\beta_i\|_1^2\Bigr\}
    \\
    &=\argmin_{\ti\beta_1,\dots,\ti\beta_n} \summ i1n \Bigl\{ \summ j1m (y_{ij}-x_{ij}\t\beta_i)^2
    + \lm_n \|\ti\beta_i\|_1^2\Bigr\}.
  }

\begin{theorem}
\label{th:lassoes1} Let $\beta_{i0}$, $i=1,\dots,n$ be $n$ vectors
and let $C_n=n^{-1}\summ i1n
\ti\beta_{i0}\t\ti\Sig_i\ti\beta_{i0}$. Let $c_n=n^{-1}\summ i1n
\min_\beta\ti\beta\t\ti\Sig_i\ti\beta$.  Then
 \eqsplit{
     \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    \leq
     \summ i1n \ti\beta_{i0}\t\ti \Sig_i \ti\beta_{i0}
    + (\frac{\lm_n} m+\del_n) \summ i1n \|\ti\beta_{i0}\|_1^2
    - (\frac {\lm_n} m-\del_n) \summ i1n \|\tihat\beta_{i}\|_1^2,
  }
where $\del_n=\max_i\|\ti S_i-\it\Sig_i\|_\en$.  If also $\lm_n/m\to0$ and $\lm_n/(m^{1/2}\log(np))\to\en$, then
 \eqsplit[bndthb]{
    \summ i1n\|\tihat\beta_i\|_1^2
    =\O_p\bigl(mn\frac{C_n-c_n}{\lm_n}\bigr) + \bigl(1+\O(\frac{m^{1/2}}{\lm_n}\log(np))\bigr)
    \summ i1n\|\ti\beta_{i0}\|_1^2
  }and
 \eqsplit{
     \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    \leq
     \summ i1n \ti\beta_{i0}\t\ti \Sig_i \ti\beta_{i0}
    + \bigl(1+\o_p(1)\bigr)\frac{\lm_n} m \summ i1n \|\ti\beta_{i0}\|_1^2.
  }
\end{theorem}


The  theorem is useful when there are vectors
$\beta_{10},\dots,\beta_{n0}$ with low $L_1$ norm which are good
approximation to the minimizers of $\ti\beta\t\ti\Sig_i\ti\beta$.
The result is meaningful, although not as strong as may be wished,
as long as $C_n-c_n\to 0$, while $n^{-1}\summ i1n
\|\ti\beta_{i0}\|_1^2=\o_p(m^{1/2})$. Of course, if the minimizer
of $\ti\beta\t\ti\Sig_i\ti\beta$ itself is sparse, then by
\eqref{bndthb} $\tihat\beta_1,\dots,\tihat\beta_n$ are as sparse
as the true minimizers (sparse in the sense of $\ell_1$ norm).

Also  note, that the prescription that the theorem gives for
selecting $\lm_n$, is sharp: choose $\lm_n$ as close as possible
to $m\del_n$, or slightly larger than $\sqrt m$.


\subsection{A Bayesian perspective}
The estimators $\tihat\beta_1,\dots,\tihat\beta_m$ look as if they
are the mode of the a-posteriori distribution of the $\beta_i$'s
when $y_{ij}|\beta_i\dist N(x_{ij}\t\beta_i,\sig^2)$, the
$\beta_1,\dots,\beta_n$ are a priori independent, and $\beta_i$
has a prior density proportional to
$\exp(-\lm_n\|\ti\beta_i\|_1^2/\sig^2)$. This distribution can be
constructed  as follows. Suppose $T_i\dist N(0,\lm_n^{-1}\sig^2)$.
Given $T_i$, let $u_{i1},\dots,u_{ip}$ be distributed uniformly on
the simplex $\{u_{i\ell}\geq 0, \summ \ell1n u_{i\ell}=|T_i|\}$.
Let $s_{i1},\dots,s_{ip}$ be \iid Rademacher random variables
(taking values $\pm 1$ with probabilities $0.5$), independent of
$T_i,u_{i1},\dots,u_{ip}$. Finally let $\beta_{i\ell}=u_{i\ell}
 s_{i\ell} $, $\ell=1,\dots,p$.

However, this  point of view is not consistent with the conditions
of Theorem \ref{th:lassoes1}. The permitted range of $\lm_n$ does
not depend on the assumed range of $\|\ti\beta_i\|$, but quite
artificially should be in the order between $m^{1/2} $ and $m$.
That is, the penalty should be increased with the number of
observations on $\beta_i$, although in a slower rate than $m$. In
fact, it goes in the `wrong' direction.  As $m\to\en$, one may
wish to use weaker a-priori  assumptions, and permits  $T$ to have
a-priori second moment going to infinity, not to 0, as entailed by
$\lm_n\to 0$.

%NB
 We would like to consider a more general penalty of the form $\summ i1n \|\beta_i\|_1^\al$. A power $\al\neq 1$ of $\ell_1$ norm of $\beta$ as a
penalty introduces a priori dependence between the variables which
is not the case for the regular lasso penalty with $\al=1$, where
all $\beta_{ij}$ are a priori independent. As $\al$ increases, the
sparsity of the different vectors tends to be the same. Note that
given the value of $\lm_n$, the $n$ problems are treated
independently.  The compound decision problem is reduced to
picking a common level of penalty. When this choice is data based,
the different vectors become dependent. This is the main benefit
of this approach---the selection of the regularization is based on
all the $mn$ observations.


For a proper Bayesian perspective, we need to consider a prior with much smaller tails than the
normal. Suppose for simplicity that $c_n=C_n$ (that is, the ``true'' regressors are sparse), and
$\max_i\|\beta_{i0}\|_1<\en$.

\begin{theorem}
\label{th:lassoes2}
Let $\beta_i$ be the minimizer of $\ti\beta\t\Sig_i\ti\beta$. Suppose $\max_i\|\beta_{i0}\|_1<\en$. Consider the estimators:
 \eqsplit[lassoesAl]{
    (\dacc\ti\hat\beta_i,\dots,\dacc\ti\hat\beta_n)
    &=\argmin_{\ti\beta_1,\dots,\ti\beta_n} \Bigl\{m\summ i1n \ti\beta_i\t\ti S_i\ti\beta_i
    + \lm_n \summ i1n \|\ti\beta_i\|_1^\al\Bigr\}
  }
for some $\al>2$. Assume that $\lambda =\O(m \delta_m) =
\O(m^{1/2} \log p)$. Then
 \eqsplit{
    n^{-1}\summ i1n \|\tihat\beta_i\|_2^2 &= \O((m\del_n/\lm_n)^{2/(\al-2)} ),
  }
and
 \eqsplit{
    \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    &\leq   \summ i1n \ti\beta_{i0}\t\ti \Sig_i \ti\beta_{i0}
    + \O_p(n (m/\lm_n)^{2/(\al-2)} \del_n^{\al/(\al-2)}).
  }

\end{theorem}

\begin{remark}\label{rem:lassoes2} If the assumption $\lambda =\O(m \delta_m)$ does not hold, i.e. if $m \delta_m/\lambda =\o(1)$, then the
error term dominates the penalty and we get similar rates as in
Theorem~\ref{th:lassoes1}, i.e.
 \eqsplit{
    n^{-1}\summ i1n \|\tihat\beta_i\|_2^2 &= \O(1),
  }
and
 \eqsplit{
    \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    &\leq  \summ i1n \ti\beta_{i0}\t\ti \Sig_i \ti\beta_{i0}
    + \O_p\left( n\lm_n/m\right).
  }

\end{remark}

 Note that we can take in fact $\lm_n\to 0$, to accommodate an increasing value of the $\tihat\beta_i$'s.

The  theorem suggests a simple way to select $\lm_n$ based on the
data. Note that $n^{-1}\summ i1n \|\tihat\beta_i\|_1^2$ is a
decreasing function of $\lm$. Hence, we can start with a very
large value of $\lm$ and decrease it until $n^{-1}\summ i1n
\|\tihat\beta_i\|_1^2\approx \lm^{-2/\al}$.

%\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> SEBAsecRINGS.tex <==


\begin{comment}
\subsection{The RINGS lasso}

Also, by analogy to the lassoes procedure, we can consider the
RINGS lasso estimator:
 \eqsplit[penRINGS]{
     \hat\scb &= \argmin_{\scb\in\R^{p\times n}}\{\summ i1n
    (y_{ij}-x_{ij}\t\beta_i)^2+\lm|||\scb|||_1^{\al}\}.
  }

Then we have the following persistency results.


\begin{theorem}\label{th:persistRINGS}

Assume that $L_F(\scb)- L_F(\scb_F^*) = \O\left(\frac p n
\sqrt{\frac{\log(pn)}{m}}
 \right)$, $|||\scb|||_1$ is bounded. Let $\hat\scb$ - solution of the RINGS
 lasso \eqref{penRINGS}.

Then, we have the following results with high probability.

1. $\alpha = 2$, $\lm \gg pm\delta_n$, then \eqsplit{
|||\hat\scb|||_1 &\leqslant \frac{\lm n}{p\delta} (L_F(\scb)-
L_F(\scb_F^*)) + \left(1 +
\O\left(\frac{pn\delta}{\lm}\right)\right)
|||\scb|||_1,\\
    \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
    &\leq   \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    + 2(\frac{\lm_n}m +p\del_n) ||| \scb|||_1^2
    + \lm n(1-  \frac{\lm_n}{m p \del_n}) \left(  L_F(\scb)-
L_F(\scb_F^*) \right)
         +2n\del_n.
 }


2. $\alpha > 2$, $\lm \ll pm\delta_n$. Then, \eqsplit{
|||\hat\scb|||_1 &\leqslant \min(n,p) \O \left(
\left(\frac{\lm}{mp\delta_n}\right)^{1/(\al-2)} \right),\\
 \summ i1n \tihat\beta_{i}\t\ti \Sig_i \tihat\beta_{i}
&\leqslant \summ i1n \ti\beta_{i}\t\ti \Sig_i \ti\beta_{i}
    +   \O((p+n) \del_n)+ p \del_n [\min(n,p)]^2 \O \left(
\left(\frac{\lm}{mp\delta_n}\right)^{2/(\al-2)} \right).
  }

% with probability at least $1 - \eta$, for any $\eta\in (0,1)$.

\end{theorem}
\end{comment}

==> SEBAsecSpectralTMP.tex <==

\section{The spectral penalty}
\label{sec:spectral}


Let \(A=\sum c_i x_ix_i\t\), be a positive semi-definite matrix,  where \(x_1,x_2,\dots\) is an orthonormal basis of eigenvectors. Then, we define \(A^{\gamma}=\sum c_i^{\gamma} x_ix_i\t\).
We consider now as penalty the function
 \eqsplit{
    \psi(\scb)=\psi(\beta_1,\dots,\beta_n)= \trace\Bigl\{\bigl(\summ i1n \beta_i\beta_i\t\bigr)^{1/2}\Bigr\}.
  }  Note that \(\psi(\scb)=\sum c_i^{1/2}\) where \(c_1,\dots,c_p\)  are the eigenvalues of \(\scb\scb\t=\summ i1n \beta_i\beta_i\t\) (including multiplicities).

\begin{lemma}
\label{lem:psiConvex}

\(\psi\) is a convex function.
\end{lemma}

In this section we study the estimator defined by
 \eqsplit{
    (\hat\beta_1,\dots,\hat\beta_n)&= \argmin_{(\beta_1,\dots,\beta_n)\in\R^{p\times n}}\{\summ i1n (y_{ij}-x_{ij}\t\beta_i)^2+\lm\psi(\beta_1,\dots,\beta_n)\}
  }

The lassoes penalty considered primary the columns of \scb. The main focus of the group lasso was the rows. The spectral penalty is symmetric in its treatment of the rows and columns since $\spect\scb =\spect\scb\t$, where $\spect A$ denotes the spectrum of $A$. Moreover, the penalty is invariant to the rotation of the matrix \scb. In fact, \(\psi(\scb) = \psi(T\scb U )\), where \(T\) and \(U\) are \(n\times n\) and \(p\times p\) rotation matrices:
 \eqsplit{
    (T\scb U)\t (T\scb U) &= U\t\scb\t\scb U
  }
and the RHS have the same eigenvalues as \(\scb\t\scb=\sum \beta_i\beta_i\t\).

Now, the standard notion of sparsity, as captured by the $L_0$ norm, or by the standard lasso and group lasso, is basis dependent. Consider the nonparametric setup in which $y_{ij} = g(z_{ij}) + \eps_{ij}$, where $z\in[0,1]$. The model fits the regression setup, if $x_{ij\ell}=h_\ell(z_{ij}$. If, for example, $g(z)=\ind(a<z\le b)$, then this example is sparse when $h_\ell(z)=\ind(z>\ell/p)$. It is not sparse if
$h_\ell(z)=(z-\ell/p)^*$. On the other hand a function $g$ which has a piece-wise constant slope is sparse in the latter basis, but not in the former.

The spectral penalty aims at finding a basis in which $\beta_1,\dots,\beta_n$ have the same pattern of sparsity. This is meaningless if $n$ is small --- any function is sparse in some basis. However, we will argue that this can be done when $n$ is large. We have






\begin{theorem}
\label{th:sparseSpect}
Suppose that for some rotation matrix $U$, and
 \eqsplit{
   \ti x_{ij\ell}=\summ l1p x_{ijl} U_{l\ell},\quad i=1,\dots,n,\; j=1,\dots,m, \;\ell=1,\dots,p,
  } 
there are  $\hat\gamma_1,\dots,\hat\gamma_n$ such that $\hat\gamma_{i\ell}=0$ for $i=1,\dots,n$ and $\ell\not\in S\subset\{1,\dots,p\}$, and
 \eqsplit{
    |\sum_j \ti x_{ij\ell}(y_{ij} - \ti x_{ij}\t \hat\gamma_{i})| 
    & \leq \lambda\bigl(1 - \hat\gamma_i\t \Bigl(\sum_k \hat\gamma_k\hat\gamma_k\t\Bigr)^{-1} \hat\beta_i \bigr)^{1/2}
    \\
    \hat\gamma_{i\ell}&=0,\quad
    i=1,\dots,n,\;\ell\not\in S\subset\{1,\dots,p\},
  }


\end{theorem}
Roughly speaking the theorem states that if the data were generated by a sparse model (in \emph{some} basis), that is with $\gamma$ whose most entries are very close to 0, and a few are well above the noise level, then the solution for the spectral penalty will have the same type of sparsity.



We consider now the penalty for $\beta_k$ for a fixed $k$. Let $A=n^{-1}\sum_{k\ne i} \beta_k\beta_k\t$.  Using Taylor expansion for not too big $\beta_i$,  based on \eqref{eigender} we get
\eqsplit{
    \trace\bigl( (nA+\beta_i\beta_i\t)^{1/2}\bigr)
     &= \sqrt{n}\trace(A^{1/2}) + \summ j1p \frac{x_j\t \beta_i\beta_i\t x_j}{2 c_j^{1/2}}
     \\
    &= \sqrt{n}\trace(A^{1/2}) + \frac 12 \beta_i\t \bigl(\sum c_j^{-1/2} x_jx_j\t\bigr)\beta_i
    \\
    &= \sqrt{n}\trace(A^{1/2}) + \frac12 \beta_i\t A^{-1/2}\beta_i
}
So, this like $\beta_i$ has a prior of $\normal(0, n \sig^2/\lm A^{1/2})$. Note that the prior is only related to the estimated variance of $\beta$. $A$ appears with the prior of $1/2$. Now $A$ is not really the estimated variance of $\beta$, only the variance of the estimates, hence it should be inflated, and the square root takes care of that. Finally, note that eventually, if $\beta_i$ is very large relative to $nA$, then the penalty become $\|\beta\|$, so the ``prior'' becomes essentially normal, but with exponential tails.

A better way to look on the penalty from a Bayesian perspective is to consider it as prior on the \(n\times p\) matrix \(\scb=(\beta_1,\dots,\beta_n)\). Recall that the penalty is invariant to the rotation of the matrix \scb. In fact, \(\psi(\scb) = \psi(T\scb U )\), where \(T\) and \(U\) are \(n\times n\) and \(p\times p\) rotation matrices. Now, this means that if \(\chi_1,\dots,\chi_p\) are orthonormal set of eigenvectors of \(\scb\t\scb\) and \(\gamma_{ij}=\chi_j\t\beta_i\) --- the PCA of \(\beta_1,\dots,\beta_n\), then \(\psi(\scb) = \summ j1p \bigl(\summ i1n \gamma_{ij}^2\bigr)^{1/2} \) --- the rms penalty in terms of the principal components. The ``prior'' is then
 \eqsplit{
    \varpropto e^{-\lm \summ j1p \|\gamma_{\cdot j}\|_2}
  }
Which is as if:
\begin{enumerate}%[(i)]
\item
Sample \(r_1,\dots,r_p\) independently from \(\Gamma(n,\lm)\) distribution.
\item
For each \(j=1,\dots,p\) sample \(\gamma_{1j},\dots,\gamma_{nj}\) independently and uniformly on the sphere with radius \(r_j\).
\item
Sample an orthonormal base \(\chi_1,\dots,\chi_p\) "uniformly''.
\item
Construct \(\beta_i = \summ j1p \gamma_{ik}\chi_k\).
\end{enumerate}
So hopefully the rms penalty ensures that the solution will be sparse in \emph{some} basis. Or the assumption (and hope) is that the Procrustes's distance between the true \(\beta\)'s and a sparse solution is small.

\subsection{Algorithm and small simulation study}

%\begin{figures}
\twofigures[1.1]{NB03042009a.eps}{NB03042009b.eps}{Component
variances and eigenvalues, \(m=25\), \(n=150\) }{fig1}
%\end{figures}

A simple algorithm is the following:
\begin{enumerate}%[(i)]
\item Initiate some small value of \(\hat
\beta_1,\dots,\hat\beta_n\). Let \(A=\summ j1n
\hat\beta_j\hat\beta_j\t\). Fix  \(\gamma\in(0,1]\), \(\eps>0\),
\(k\), and \(c>1\). \item\label{A1st1} For \(i=1,\dots,n\):
\begin{enumerate}%[(i)]
\item Compute \(\delta_i = (X_i\t X_i + \lm A^{-1/2})^{-1}X_i\t
(y_i-X_i\hat\beta_i)\). \item Update \(A\leftarrow
A-\hat\beta_i\hat\beta_i\);
\(\hat\beta_i\leftarrow\hat\beta_i+\gamma\delta_i\); \(A\leftarrow
A+\hat\beta_i\hat\beta_i\);
\end{enumerate}
\item if \(\summ j1p \ind\bigl(n^{-1}\summ
i1n\hat\beta_{ij}^2>\eps\bigr)>k \) update
\(\lambda\leftarrow\lambda c\) otherwise
\(\lambda\leftarrow\lambda/ c\). \item Return to step \ref{A1st1}
unless there is no real change of coefficients.
\end{enumerate}

Comment: to fasten the computation, the SVD was computed only
every 10 values of \(i\).

As a simulation we applied the above algorithm to the following
simulated data  (\textbf{NB05Apr2009.m}).. We generated random
\(\beta_1,\dots,\beta_{150}\in\R^{150}\) such that all coordinates
are independent, and \(\beta_{ij}\dist\normal(0, e^{-2j/5})\). All
\(X_{ij\ell}\) are \iid \(\normal(0,1)\), and \(y_{ij} =
x_{ij\cdot}\t \beta_i+\eps_{ij}\), where \(\eps_{ij}\) are all
\iid \(\normal(0,1)\).  The true \(R^2\) obtained was
approximately  0.73. The number of replicates per value of
\(\beta\), \(m\), varied between 5 to 300. We consider two
measures of estimation error:
 \eqsplit{
    L_{\rm par} &= \frac{\summ i1n \|\hat\beta_i-\beta_i\|_\en} {\summ i1n \|\beta_i\|_\en}
    \\
    L_{\rm pre}  &= \frac{\summ i1n \|X_j(\hat\beta_i-\beta_i)\|_\en} {\summ i1n \|X_i\beta_i\|_\en}
  }


%\begin{figures}
\onefigure[1.1]{NB11Apr2009d.eps}{ Lower lip position while
repeating 32 times 'Say bob again'}{fig2}
%\end{figures}

The algorithm stopped after 30--50 iterations. Figure \label{fig1}
is a graphical presentation of a typical result. A summary is
given in Table \ref{tab1}. Note that \(m\) has a critical  impact
on the estimation problem. However, with as little as \(5\)
observations per \(R^{150}\) vector of parameter we obtain a
significant reduction in the prediction error.
\begin{table}[H]
\caption{\label{tab1}The estimation and prediction error as
function of the number of observations per vector of parameters
Means (and SDK).}
\begin{center}

\begin{tabular}{|r|r|r|}
\hline
$m$     &   \(L_{\rm par}\)  & $L_{\rm pre}$    \\
\hline\hline
5  &    0.9530 (0.0075)               &   0.7349 (0.0375)         \\
\hline
25  &   0.7085 (0.0289)                &  0.7364 (0.0238)           \\
\hline
300  &  0.2470 (0.0080)                 &  0.5207 (0.0179)          \\
\hline

\end{tabular}
\end{center}
\end{table}


%\begin{figures}
\threefiguresV[1.5]{NB11Apr2009a.eps}{NB11Apr2009b.eps}{NB11Apr2009c.eps}{Eigenvalue,
coefficient variance and typical observed and smooth path.}{fig3}
%\end{figures}

The technique is natural for functional data analysis. We used the
data LipPos taken James O. Ramsay and Bernard W. Silverman
http://www.stats.ox.ac.uk/~silverma/fdacasebook/lipemg.html. The
data is described in Figure \ref{fig2}. However we added noise to
the data as will be seen in Figure \ref{fig3}. The position is
measured at $m=501$ time points, with \(n=32\) repetitions.


As the matrix \(X\) we considered the union of 6 cubic spline
bases with, respectively, 5, 10, 20, 100, 200, and 500 knots
(i.e., \(p=841\), and \(X_i\) does not depend on \(i\)). A
Gaussian noise with \(\sigma=0.001\) was added to \(Y\). The
result of the analysis is given in Figure \ref{fig3}. Figure
\ref{fig4} present the projection of the mean path on the first
eigen-vectors of \(\summ i1n \hat\beta_i\hat\beta_i\t\). (Analysis
done using NB11Apr2009.m).


%\begin{figures}
\onefigure[0.5]{NB11Apr2009e.eps}{Projection of the estimated mean
path on the 2 first eigen-vectors of \(\summ i1n
\hat\beta_i\hat\beta_i\t\) and the true mean path.}{fig4}
%\end{figures}

The final example we consider is some what arbitrary. The data,
taken from StatLib, is of the daily wind speeds for 1961-1978 at
12 synoptic meteorological stations in the Republic of Ireland. As
the \(Y\) variable we considered one of the stations (station
BIR). As explanatory variables we considered the 11 other station
of the same day, plus all 12 stations 70 days back (with the
constant we have altogether 852 explanatory variables). The
analysis was stratified by month. For simplicity, only the first
28 days of the month were taken, and the first year, 1961, served
only for explanatory purpose. The last year was served only for
testing purpose, so, the training set was for 16 years (\(N=12\),
\(m=448\), and \(P=852\) ).  In Figure \ref{fig5} we give the 2nd
moments of the coefficients and the scatter plot of predictions
vs. true value of the last year. (Analysis done using
NB14Apr2009.m)

%\begin{figures}
\twofigures[0.75]{NB14Apr2009a.eps}{NB14Apr2009b.eps}{Coefficient
2nd moment and prediction vs.true value of the test year.}{fig5}
%\end{figures}

\subsection{Fixed design matrix }

We start with the simple case where \(X_i=\ti X\), that is
\(y_i=X\beta_i+\eps_i\), \(i=1,\dots,n\), where \(y_i,\eps_i\in
\R^m\) and \(\beta_i\in\R^p\). The general approach for sparsity
depends heavily on representing the model in the proper base, the
one in which sparsity is attained. That is the base in which there
is a sparse approximation of the regression function. This isn't
the case with the rms penalty.  The penalty function is invariant
to rotation, \(\psi(\beta_1,\dots,\beta_n)
=\psi(T\beta_1,\dots,T\beta_n)\) where \(T\) is a matrix with
orthonormal columns, \(T\t T=I_p\), hence, the prediction
\(X\hat\beta_i\) is invariant for a rotation of the design matrix,
such that the model is equivalent to \(Y_i=\ti X\beta_i+\eps_i\),
where \(\ti X=XT\t\). This means that sparsity will be in the
right base.


\subsection{The spectral penalty: 2D case}

In the 2-dimensional case ($p=2$), we can find the explicit
expression for the penalty in terms of $\beta_{\cdot \ell}$. The
eigenvalues of
 \eqsplit{
     \scb \scb\t = \begin{pmatrix}  ||\beta_{\cdot 1}||_2^2 & \langle \beta_{\cdot 1}, \beta_{\cdot 2}\rangle  \\ \langle \beta_{\cdot 1}, \beta_{\cdot 2}\rangle & ||\beta_{\cdot 2}||_2^2 \end{pmatrix}
%    &= \sigma\begin{pmatrix} \sum_i \ti\beta_i\ti\beta_i\t &  0 \\ 0 & t^2\sum b_i^2 - t^2\sum_i b_i\ti\beta_i\t \Bigl(\sum_i \ti\beta_i\ti\beta_i\t\Bigr)^{-1} \sum_ib_i\ti\beta_i \end{pmatrix} \\
%    &= \sig\Bigl(\sum \ti\beta_i\ti\beta_i\t\Bigr) \union t^2 \bigl(\sum b_i^2 - \sum_i b_i\ti\beta_i\t \Bigl(\sum_i \ti\beta_i\ti\beta_i\t\Bigr)^{-1} \sum_ib_i\ti\beta_i \bigr)
  }
are the solutions of $(||\beta_{\cdot 1}||_2^2 - z)(||\beta_{\cdot
2}||_2^2 - z) - \langle \beta_{\cdot 1}, \beta_{\cdot
2}\rangle^2=0$, i.e. are
$$
z_{1,2} = \frac 1 2 \left[ ||\beta_{\cdot 1}||_2^2 +
||\beta_{\cdot 2}||_2^2 \pm \sqrt{ \left(||\beta_{\cdot 1}||_2^2 -
||\beta_{\cdot 2}||_2^2\right)^2 + 4 \langle \beta_{\cdot 1},
\beta_{\cdot 2}\rangle^2} \right],
$$
and hence it can be shown that
$$
\psi(\scb) =z_1^{1/2}+ z_2^{1/2} = \sqrt{||\beta_{\cdot 1}||_2^2 +
||\beta_{\cdot 2}||_2^2 + 2 \sqrt{||\beta_{\cdot 1}||_2^2
||\beta_{\cdot 2}||_2^2 - \langle \beta_{\cdot 1}, \beta_{\cdot
2}\rangle^2}}
$$
due to identity $\sqrt{A + \sqrt{A^2-4B}} + \sqrt{A -
\sqrt{A^2-4B}} = \sqrt{2A +4\sqrt{B}}$.

Hence, in the directions where $\beta_{\cdot 1}$ and $\beta_{\cdot
2}$ are orthogonal, $\psi(\scb)$ behaves like $\ell_1$ penalty,
and in the directions they are collinear ($\langle \beta_{\cdot
1}, \beta_{\cdot 2}\rangle = \pm 1$) $\psi(\scb)$ behaves like
$\ell_2$ penalty.

If the ``correlation'' between $\beta_{\cdot 1}$ and $\beta_{\cdot
2}$ is $\rho=\frac{\langle \beta_{\cdot 1}, \beta_{\cdot
2}\rangle}{||\beta_{\cdot 1}||_2 ||\beta_{\cdot 2}||_2}$, then the
penalty ``ball'' (curve as a function of $||\beta_{\cdot 1}||_2$
and $||\beta_{\cdot 2}||_2$) is plotted for different values of
$\rho$ (Figure \ref{figBall}).

%\begin{figures}
\onefigure[0.7]{SpectBall.eps}{ Spectral ``ball'' as a function of%$||x|| = ||\beta_{\cdot 1}||_2$ and $||\beta_{\cdot 2}||_2$ given
different values of $\rho$. }{figBall}
%\end{figures}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{ Equations for $\widehat{\beta}$.}


Differentiating the ``loss'' with respect to $\beta_{ij}$, we
obtain the equations for $\widehat{\beta}$:
$$
2\sum_{j} x_{ij\ell} (Y_{ij} - x_{ij\cdot }\t \widehat{\beta}_i) =
\lambda \, \sgn(\widehat{\beta}_{i\ell}) \left( 1 -
\widehat{\beta}_{i L}\t (\sum_{k} \widehat{\beta}_{k L}
\widehat{\beta}_{k L}\t)^{-1} \widehat{\beta}_{i L} \right)^{1/2},
$$
if $\widehat{\beta}_{i\ell} \neq 0$, and if
$$
|2\sum_{j} x_{ij\ell} (Y_{ij} - x_{ij\cdot }\t \widehat{\beta}_i)|
\leqslant  \lambda  \left( 1 - \widehat{\beta}_{i L}\t (\sum_{k}
\widehat{\beta}_{k L} \widehat{\beta}_{k L}\t)^{-1}
\widehat{\beta}_{i L} \right)^{1/2},
$$
$\widehat{\beta}_{i\ell} = 0$. Here $L = J(\beta) \setminus
\{\ell\}$, i.e. we assume that $\exists (\sum_{k}
\widehat{\beta}_{k L} \widehat{\beta}_{k L}\t)^{-1}$. Does it
always? If not, how does the expression changes then?

\subsection{ Equations for $\widehat{\gamma}$.}

If we parameterize $\beta_i = U\t \gamma_i$, the equations for
$\gamma$ become:
$$
\sum_{jk} x_{ijk} U_{\ell k} (Y_{ij} - X_{ij}\t U\t \gamma_i ) =
\frac {\lambda}{2} \frac{\gamma_{i\ell}}{ ||\gamma_{\cdot
\ell}||_2},
$$
if $\gamma_{i\ell} \neq 0$, and
$$
|\sum_{jk} x_{ijk} U_{\ell k} (Y_{ij} - X_{ij}\t U\t \gamma_i )|
\leqslant \frac {\lambda}{2} \frac{|\gamma_{i\ell}|}{
||\gamma_{\cdot \ell}||_2},
$$
$\gamma_{i\ell} = 0$.


\subsection{The spectral penalty: inequalities}

%[assumption: $X_{i\cdot \ell}X_{i\cdot \ell}\t =C$, for all $i$ and $\ell$. ]

If $\beta\beta\t = U C U\t$ and $\hat\beta\hat\beta\t = \hat{U}
\hat{C} \hat{U}\t$ where $\hat\beta$ is the solution of the
spectral RMS problem \eqref{rotatedlassostar}. Then $U\t\hat\beta$
is the solution of the standard RMS (group lasso) problem
\eqref{lassostar} with $\tilde{X}_i = U^T X_i$. Hence,
Lemma~\ref{lem:GroupLasso} is satisfied for $\gamma = U\t\beta$
and ``estimate'' $\tilde\gamma = U\t\hat\beta$ with design
matrix $\tilde{X}$.

Note that even if $\beta$ and $\hat\beta$ are close, $\gamma$ and
$\hat\gamma = \hat{U}\t\hat\beta$ are close only up to a
permutation of variables. Hence, we will be interested in
comparing $U\t\hat{U}$ to a permutation matrix (e.g. testing that
 all eigenvalues are close to $\pm 1$).

We may be interested in sparsity of $\beta$ and $\gamma$, as well
as the approximation error of estimating $f$ and $\beta$. Thus, we
obtain the following results.

\begin{lemma}\label{lem:RotateGroupLasso}
Let \(Y_{ij}\dist \normal (f_{ij},\sig^2)\) independent,
\(f_{ij}=x_{ij}\t\beta_i\), \(x_{ij}\in \R^p\),
\(\beta_i\in\R^p\), \(i=1,\dots,n\), \(j=1,\dots,m\).  Consider
 \eqsplit[rotatedlassostar]{
    (\hat\beta_1,\dots,\hat\beta_n) &=
    \argmin \Biggl[ \summ i1n \summ j1m (Y_{ij} - x_{ij}\t\,\beta_i)^2 + \lambda
   \trace  \Bigl\{ \summ i1n \beta_{i }\beta_i^T\Bigr\}^{1/2}
   \Biggr],
  }
with \(\lm=4A\sig\tilde\Lm_x\sqrt{n \log(pn)}\), where
\(\tilde\Lm_x=  \max_{i}\sqrt{\sum_{\ell,j} x_{i j \ell}^2 }\) and
\(A>\sqrt2\).

Then, with probability at least \(1-(np)^{1-A^2/2}\):  % \mu=\sig A\bigl(\log(np)\bigr)
\begin{enumerate}[a)]

\item \(\forall \beta\in\R^{p\times n}\):%
     \eqsplit[SPECTboundf_beta1]{ %
     \|f-\hat f\|_2^2 +  \frac{\lm}{2\sqrt{n}}  \summ {\ell}1p
      \summ i1n |\gamma_{i\ell} - (U\t\hat{U})_\ell
       \hat\gamma_{i}| \le \|f - f_{\scb}\|_2^2
     +  \lm (1/\sqrt{n}+1)  \sum_{\ell\in J( \gamma)}\|\hat\gamma_{\cdot\ell}
     - (U\t\hat{U})_\ell \hat\gamma\|_1,
     } %
where \(f_{\scb ij} = x_{ij}\t\beta_i = x_{ij}\t U\t \gamma_i \),
%$\lambda = 4\sqrt{n}\max_i \sqrt{\sum_j c_{ij}^2}$
 and%
 \eqsplit{
J(\gamma)=\Bigl\{\ell\in\{1,\dots,p\}:\summ i1n\gamma_{i\ell}^2>0\Bigr\}. %
 }

\item \(\forall \beta\in\R^{p\times n}\):%
     \eqsplit[SPECTboundf_beta1]{ %
     \|f-\hat f\|_2^2 +  \lm/2  \summ {\ell}1p
      \summ i1n |\gamma_{i\ell} - (U\t\hat{U})_\ell \hat\gamma_{i}| \le \|f - f_{\scb}\|_2^2
     + 2\lm \sum_{\ell\in J( \gamma)}\|\hat\gamma_{\cdot\ell}
     - \gamma_{\cdot\ell}\|_2.
     } %

\item Let $\tilde\gamma = U\t\hat\beta$ and
    \(\scm(\tilde\gamma) = |J(\tilde\gamma)|\) be the number of
    non-zero coefficients of \(\tilde\gamma\),
then \eqsplit{ \scm(\tilde\gamma) \leq  \|f-\hat f\|_2^2  \frac{m
p }{15\sig^2 A^2 n\log(np)}. }

\item (Do a bound on $U\t\hat{U} - P$, $P$ - a permutation)
%$\scm(\beta)$

\end{enumerate}
\end{lemma}

Note that for any $p\geqslant 1$,
$$
 ||\beta_i - \hat\beta_{i}||_p \leqslant ||U||_p
||\gamma_i - U\t\hat{U}\hat\gamma_{i}||_p,
$$
and for $p=2$,
$$
||\beta_i - \hat\beta_{i}||_2 = ||\gamma_i -
U\t\hat{U}\hat\gamma_{i}||_2.
$$


\begin{proof}


%Also, the random term can be bounded with probability at least
%$1-(np)^{1-A^2/2}$ as

Similarly to the proof of Lemma~\ref{lem:GroupLasso}, we have
 \eqsplit{
 \|f-\hat f\|_2^2  & = \|f_{\beta}-f\|_2^2
    +2\sum_{ij}\eps_{ij}x_{ij}\t(U \gamma_i - \hat{U}\hat\gamma_i).
  }
The last term can be bounded with high probability. Using
inequality $|a\t A b| \leqslant ||A||_2\, ||a||_2\, ||b||_2$, we
obtain
 \eqsplit{
&|\sum_j \eps_{ij}x_{ij}\t(U \gamma_i -\hat{U}\hat\gamma_i)|
\leqslant \| \sum_j\eps_{ij}x_{ij}\t \|_2 \left[ \|U \gamma_i
-\hat{U}\hat\gamma_i\|_2 \right] \leqslant  \sqrt{\sum_j c_{ij}^2
} \left[ \| \gamma_i -U\t\hat{U}\hat\gamma_i\|_2 \right].
 }

Note that on one hand,
 \eqsplit{
 & \sum_{ij}  c_{ij} | \beta_{ij} - \hat\beta_{ij}|
  = \sum_{ij}  c_{ij}    | U_j\t \gamma_{i} - \hat{U}_j\t\hat\gamma_{i}|
  \\
&\leqslant \sum_{i} \sqrt{\sum_j c_{ij}^2}  \|  U\t \gamma_{i} -
\hat{U} \t\hat\gamma_{i}\|_2 = \sum_{i} \sqrt{\sum_j c_{ij}^2} \|
\gamma_{i} - U\hat{U} \t\hat\gamma_{i}\|_2\\
& \leqslant \max_i \sqrt{\sum_j c_{ij}^2} \sum_{\ell} \|
\gamma_{\cdot \ell} - (U\t\hat{U})_{\ell} \hat\gamma\|_1\\
&\leqslant \sqrt{n} \max_i \sqrt{\sum_j c_{ij}^2} \sum_{\ell} \|
\gamma_{\cdot \ell} - (U\t\hat{U})_{\ell} \hat\gamma\|_2
 }

On the other hand,
 \eqsplit{
 & \sum_{ij}  c_{ij} | \beta_{ij} - \hat\beta_{ij}|
  = \sum_{ij}  c_{ij}    | U_j\t \gamma_{i} - \hat{U}_j\t\hat\gamma_{i}|
  \\
&\leqslant \sum_{i} \max_j c_{ij}   \|  U\t \gamma_{i} - \hat{U}
\t\hat\gamma_{i}\|_1 \leqslant ||U\t||_1  \max_{ij} c_{ij}
\sum_{i} \|\gamma_{i} - U\t\hat{U}\hat\gamma_{i}\|_1\\
&\leqslant \sqrt{p}  \max_{ij} c_{ij} \sum_{\ell} \|\gamma_{\cdot
\ell} - (U\t\hat{U})_{\ell}\hat\gamma\|_1
 }

[can be also bounded by]
$$
2\sum_{i} \max_j c_{ij} \|U\t \gamma_{i } -
\hat{U}\t\hat\gamma_{i}\|_1 = 2\sum_{i} \sqrt{\sum_j c_{i j}^2} \|
\gamma_{i } - U \hat{U}\t\hat\gamma_{i}\|_2,
$$


a) We have that
 \eqsplit{
    \|f-\hat f\|_2^2 &+  \lm_3 \sum_{i} \|\gamma_{i} - \hat{U} U\t\hat\gamma_{i}\|_1
    \leq \|f_\scb - f\|_2^2
    +  \lm_3 \sum_i
    \|\gamma_{i}-\hat{U} U\t\hat\gamma_{i}\|_1
    +\lm\sum_\ell \|\gamma_{\cdot\ell}\|_2
    \\
    &\hspace{2em}
    -\lm\sum_\ell \| (U\t\hat{U})_\ell\hat\gamma\|_2
    + 2 \max_i \sqrt{\sum_j c_{ij}^2} \sum_{\ell i}    |\gamma_{i\ell} -
    (U\t\hat{U})_{\ell}\hat\gamma_{i} |\\
    &\leqslant \|f_\scb - f\|_2^2
    +\lm\sum_\ell \|\gamma_{\cdot\ell}\|_2
    \\
    &\hspace{2em}
    -\lm\sum_\ell \|U\t\hat{U}\hat\gamma_{\cdot\ell}\|_2
    + \sum_{\ell} \left( 2\max_i \sqrt{\sum_j c_{ij}^2} + \lm_3\right) \|\gamma_{\cdot \ell} -
    (\hat{U} U\t)_{\ell}\hat\gamma  \|_1\\ &= \|f_\scb - f\|_2^2 +
    \sum_\ell S_\ell.
  }


For $\ell \notin J(\gamma)$, we have
 \eqsplit{
S_\ell &= -\lm \|(U\t\hat{U})_\ell\hat\gamma \|_2 + \left( 2\max_i
\sqrt{\sum_j c_{ij}^2} + \lm_3\right)
\|(U\t\hat{U})_{\ell}\hat\gamma \|_1\\ &\leqslant
\|(U\t\hat{U})_{\ell}\hat\gamma \|_2 \left[ -\lm + \sqrt{n} \left(
2\max_i \sqrt{\sum_j c_{ij}^2} + \lm_3\right) \right] \leqslant 0
}
 for $\lm \geqslant \sqrt{n} ( 2\max_i \sqrt{\sum_j
c_{ij}^2} + \lm_3)$. E.g. we can take $\lm_3 = 2\max_i
\sqrt{\sum_j c_{ij}^2} = \lm/(2\sqrt{n})$.


For $\ell \in J(\gamma)$, we have
 \eqsplit{
S_\ell &\leqslant \lm \|\gamma_{\cdot\ell}-(U\t\hat{U})_{
\ell}\hat\gamma\|_2 + ( 2\max_i \sqrt{\sum_j c_{ij}^2} + \lm_3)
\|\gamma_{\cdot \ell} - (\hat{U} U\t)_{\ell}\hat\gamma  \|_1\\
&\leqslant (\lm +  2\max_i \sqrt{\sum_j c_{ij}^2} + \lm_3)
\|\gamma_{\cdot \ell} - (\hat{U} U\t)_{\ell}\hat\gamma  \|_1 = \lm
(1+1/\sqrt{n})\|\gamma_{\cdot \ell} - (\hat{U}
U\t)_{\ell}\hat\gamma  \|_1.}

Substituting the values of $\lm$ and $\lm_3$, we obtain a).

b) We have that
 \eqsplit{
    \|f-\hat f\|_2^2 &+  \lm_2 \sum_{i} \|\gamma_{i} - \hat{U}
    U\t\hat\gamma_{i}\|_2
    \leq \|f_\scb - f\|_2^2
    +  \lm_2 \sum_i
    \|\gamma_{i}-\hat{U} U\t\hat\gamma_{i}\|_2
    +\lm\sum_\ell \|\gamma_{\cdot\ell}\|_2
    \\
    &\hspace{2em}
    -\lm\sum_\ell \|U\t\hat{U}\hat\gamma_{\cdot\ell}\|_2
    + 2\sqrt{n} \max_i \sqrt{\sum_j c_{ij}^2} \sum_{\ell} \|
\gamma_{\cdot \ell} - (U\t\hat{U})_{\ell} \hat\gamma\|_2
%    \max_i \sqrt{\sum_j c_{ij}^2} \sum_{\ell i}    |\gamma_{i\ell} -
%    (U\t\hat{U})_{\ell}\hat\gamma_{i} |\\
  }
%rm can also be  \sqrt{\sum_{ij} c_{ij}^2} instead of \sqrt{n} \max_i \sqrt{\sum_j c_{ij}^2}

For $\ell \notin J(\gamma)$, we have
 \eqsplit{
S_\ell &= \|U\t\hat{U}\hat\gamma_{\cdot\ell}\|_2 [ -\lm + (
2\sqrt{n}\max_i \sqrt{\sum_j c_{ij}^2} + \lm_2)\leqslant 0 }
 for $\lm \geqslant 2\sqrt{n} \max_i \sqrt{\sum_j
c_{ij}^2} + \lm_2$. E.g. we can take $\lm_2 = 2\sqrt{n}\max_i
\sqrt{\sum_j c_{ij}^2} = \lm/2$, i.e. we can use the same $\lm$.

For $\ell \in J(\gamma)$, we have
 \eqsplit{
S_\ell &\leqslant \|\gamma_{\cdot\ell}-(U\t\hat{U})_{
\ell}\hat\gamma\|_2 (\lm +  2\sqrt{n}\max_i \sqrt{\sum_j c_{ij}^2}
+ \lm_2) = 2\lm  \|\gamma_{\cdot \ell} - (\hat{U}
U\t)_{\ell}\hat\gamma  \|_2.}

c) We apply Lemma~\ref{lem:GroupLasso} with design matrix
$\tilde{X}$. Then constant $\tilde{\Lm}_0$ is:
$$
\tilde{x}_{ij\ell}^2 = (U^T X_i)_{j\ell}^2 =  (\sum_k x_{ijk}
U_{k\ell } )^2 \leqslant  \sum_k x_{ij k}^2
  \sum_k U_{k \ell}^2 = \sum_k x_{ijk}^2.
$$
Hence,
\eqsplit{
 \Lm_0 (\tilde{X}) &\le  \frac{\sum_\ell
 \max_{ij}\tilde{x}_{ij\ell}^2}  {\lm^2 - \mu^2 \max_\ell \sum_{ij}\tilde{x}_{ij\ell}^2}
\le \frac{p \max_{ij} \sum_\ell x_{ij\ell}^2}  {16n\mu^2 \max_{i}
\sum_{\ell,j} x_{i j \ell}^2 - \mu^2
  \sum_{ij\ell} x_{ij\ell}^2}\\
&\le \frac{p \max_{ij} \sum_\ell x_{ij\ell}^2}  {15n\mu^2 \max_{i}
\sum_{\ell,j} x_{i j \ell}^2} \le \frac{p \max_{ij} \sum_\ell
x_{ij\ell}^2}  {15n\mu^2 \max_{i j} \sum_{\ell} x_{i j \ell}^2}\\
&\le \frac{p }{15n\mu^2} = \frac{p }{15\sig^2 A^2 n\log(np)}
}
 since \(\mu=\sig A\bigl(\log(np)\bigr)^{1/2}\).
\end{proof}

We need one of the following assumptions (repeated). Following
(e.g. Obozinski et al, 2008), denote $||x||_{p/q} = \summ i1n
\left[|| x_{\cdot i} ||_p^q \right]^{1/q}$, $x\in
\mathbb{R}^{m\times n}$.

\noindent{\bf Assumption URE2$_n(s; c_0)$}. For some integer $s$ such that
$1 \leqslant s \leqslant p$, and a positive number $c_0$ the
following condition holds:
\begin{equation}
\tilde{\kappa}_{U \, n}(s, c_0)^2 := \min_i \min_{\substack{J_0
\subseteq \{1,\dots,\,p\},\\ |J_0|\leqslant\, s}} \,
\min_{U\in \mathbb{R}^{p\times p}: \, U U\t = I} \min_{\substack{\delta \in \mathbb{R}^{n\times p}\setminus \{0\}, \\
 ||\delta_{ \cdot \, J_0^c}||_{2/1} \leqslant \, c_0
 ||\delta_{ \cdot \, J_0}||_{2/1}  }} \frac{|| X_{i\cdot\cdot}^T U \delta_i||_2^2}{|| \delta_{i J_0}||_2^2} > 0.
\end{equation}


\noindent{\bf Assumption MURE2$_n(s; c_0)$}. For some integer $s$ such that
$1 \leqslant s \leqslant p$, and a positive number $c_0$ the
following condition holds:
\begin{equation}
\tilde{\kappa}_{U \, n}(s, c_0)^2 := \min_{\substack{J_0 \subseteq
\{1,\dots,\,p\},\\ |J_0|\leqslant\, s}} \,
\min_{U\in \mathbb{R}^{p\times p}: \, U U\t = I} \min_{\substack{\delta \in \mathbb{R}^{n\times p}\setminus \{0\}, \\
 ||\delta_{ \cdot \, J_0^c}||_{2/1} \leqslant \, c_0
 ||\delta_{ \cdot \, J_0}||_{2/1}  }} \frac{\summ i1n ||
X_{i\cdot\cdot}^T U \delta_i||_2^2}{ \summ i1n || \delta_{i
J_0}||_2^2} > 0.
\end{equation}

% analogue of Theorem 6.1 in BRT
\begin{theorem} Let \(Y_{ij}\dist \normal (f_{ij},\sig^2)\) independent,
\(f_{ij}=x_{ij}\t\beta_i\), \(x_{ij}\in \R^p\),
\(\beta_i\in\R^p\), \(i=1,\dots,n\), \(j=1,\dots,m\), $p\geqslant
2$.  Fix some $\varepsilon  > 0$ and let Assumption MURE2$_n(s; 3
+ 4/\varepsilon)$ (or Assumption URE2$_n(s; 3 + 4/\varepsilon)$)
be satisfied for $X=(x_{ijl})$.

Consider the spectral RMS estimator $\hat{f}_{ij} =
X_{ij}\t\hat{\beta}_i$ where $\hat{\beta}$ is defined by
\eqref{rotatedlassostar} with \(\lm=4A\sig\tilde\Lm_x\sqrt{n
\log(pn)}\), where \(\tilde\Lm_x= \max_{i}\sqrt{\sum_{\ell,j} x_{i
j \ell}^2 }\) and \(A>\sqrt2\).

Then, with probability at least \(1-(np)^{1-A^2/2}\),
   \eqsplit{ %
     \|f-\hat f\|_2^2  \le (1+\varepsilon)\inf_{\substack{\beta\in\mathbb{R}^p,\\ \scm(\gamma)\le s}} \left[\|f - f_{\scb}\|_2^2
     + \scm(\gamma) n\log(np) \frac{16 A^2 \sigma^2
     \Lambda_{\tilde{x}}^2 C_{\varepsilon} }{\kappa_{2n}^2(s, 3+4/\varepsilon))}\right],
     } %
where  $C_{\varepsilon} = \frac{(\varepsilon+2)^2}{\varepsilon
(1+\varepsilon)} >0$.

Also, we can show that
   \eqsplit{ %
     \|f-\hat f\|_2  \le (1+\varepsilon) \inf_{\substack{\beta\in\mathbb{R}^p,\\ \scm(\gamma)\le s}} \left[\|f - f_{\scb}\|_2
     + 2\lambda \frac{\sqrt{\scm(\gamma)} }{\kappa (s,
     3+4/\varepsilon) )}\right].
     } %

\end{theorem}

\begin{proof}
Fix an arbitrary $\beta\in\mathbb{R}^p$ such that $\scm(\gamma)\le
s$.

On event $\sca$ defined in the proof of Lemma 1, inequalities
\eqref{boundf} hold. Consider two cases.

\begin{enumerate}
\item $2\lambda \sum_{\ell \in J(\gamma)} ||\gamma_{\cdot\ell} -
\tilde\gamma_{\cdot\ell}||_2  \leqslant \varepsilon || f -
f_{\scb}||_2^2$. In this case, the result of the theorem follows
trivially from \eqref{boundf}.

\item $\varepsilon || f - f_{\scb}||_2^2 < 2\lambda \sum_{\ell \in
J(\gamma)} ||\gamma_{\cdot\ell} - \tilde\gamma_{\cdot\ell}||_2$.
Denote the event  defined by this  inequality by $\tilde\sca$; all
subsequent inequalities hold on $\sca \cap \tilde\sca$.

On this event, we get from \eqref{SPECTboundf} that
$$
\sum_{\ell \in J^c(\gamma)}  ||\gamma_{\cdot\ell} -
\tilde\gamma_{\cdot\ell}||_2 \leqslant (3+4/\varepsilon)
\sum_{\ell \in J(\beta)} ||\gamma_{\cdot\ell} -
\tilde\gamma_{\cdot\ell}||_2.
$$
Assumption MRE$_n(s, 3+4/\varepsilon)$ (or MURE$_n(s,
3+4/\varepsilon)$, with the corresponding $\kappa$) implies that
$$
\kappa^2 \sum_{\ell \in J(\gamma)} |\gamma_{i\ell} -
\tilde\gamma_{i\ell}|_2^2 \leqslant || X_{i\cdot\cdot}\t
(\beta_{i\cdot } - \hat\beta_{i\cdot}) ||_2^2 = || f_{\rb \,
i\cdot } - \hat{f}_{i\cdot } ||_2^2,
$$
where $\kappa = \kappa(s, 3+4/\varepsilon)$.

Hence, by \eqref{SPECTboundf},
\begin{eqnarray*} %check
 \|f-\hat f\|_2^2  &\le&  \|f - f_{\scb}\|_2^2
     +2\lm \sum_{\ell\in J(\gamma)}\|\tilde\gamma_{\cdot\ell}
     -\gamma_{\cdot\ell}\|_2\\
     &\le&  \|f - f_{\scb}\|_2^2 +
     2\lm \sqrt{\scm(\gamma)} \left[\sum_{\ell\in J(\gamma)}\|\tilde\gamma_{\cdot\ell}
     -\gamma_{\cdot\ell}\|_2^2\right]^{1/2}\\
     &=&  \|f - f_{\scb}\|_2^2 +
     2\lm \sqrt{\scm(\gamma)} \left[\sum_{i=1}^n\sum_{\ell\in J(\gamma)} |\tilde\gamma_{\cdot\ell}
     -\gamma_{\cdot\ell}|_2^2\right]^{1/2}\\
     &\le&  \|f - f_{\scb}\|_2^2 +
     2\lm \sqrt{\scm(\gamma)} \left[\sum_{i=1}^n  \frac 1 {\kappa^2} \|\hat{f}_{i\cdot} - f_{\scb\, i\cdot}\|_2^2
     \right]^{1/2}\\
     &=&  \|f - f_{\scb}\|_2^2 +
     2\lm \frac{\sqrt{\scm(\gamma)}}{\kappa}   \|\hat{f}  - f_{\scb }\|_2\\
     &\le&  \|f - f_{\scb}\|_2^2 +
     2\lm \frac{\sqrt{\scm(\beta)}}{\kappa} \left[  \|\hat{f}  - f \|_2 + \|f  - f_{\scb }\|_2 \right].
\end{eqnarray*}
Using inequality $2xy \le  x^2/b +   b y^2$ with $b\in(0,1)$, $x =
\lm \sqrt{\scm(\beta)}/\kappa$, and $y$ being either $\|\hat{f}  -
f \|_2$ or $\|f  - f_{\scb }\|_2$, we can decouple the last term
to obtain
\begin{eqnarray*}
 \|f-\hat f\|_2^2 &\le& \frac{1+b}{1-b} \|f - f_{\scb}\|_2^2 +
      \frac{2 \lm^2\scm(\beta)}{b(1-b)\kappa^2}, \quad \forall b\in(0,1).
\end{eqnarray*}
Taking $b=\left(1+2/\varepsilon\right)^{-1}$ we obtain
\begin{eqnarray*}
 \|f-\hat f\|_2^2 &\le& (1+\varepsilon) \|f - f_{\scb}\|_2^2 +
      \frac{\lm^2\scm(\gamma) (\varepsilon+2)^2}{\varepsilon
      \kappa^2}.
\end{eqnarray*}
 Substituting the value of $\lm$ and taking the infimum over all considered $\beta$ finishes the proof of the theorem.
\end{enumerate}

\end{proof}


For linear regression, we obtain the following inequalities.
\begin{corollary}
\eqsplit{
 \frac 1 n \sum_{i=1}^n ||X_i\t(\beta_i -
\hat\beta_{i})||_2^2 &\leqslant \scm(\gamma) \log(np) \frac{16 A^2
\sigma^2
     \Lambda_{\tilde{x}}^2 C_{\varepsilon} }{\kappa_{2n}^2(s,
     3+4/\varepsilon)},\\
\frac 1 n \sum_{i=1}^n ||\beta_i - \hat\beta_{i}||_2^2 &\leqslant
C_x \scm(\gamma) \log(np) \frac{16 A^2 \sigma^2
     \Lambda_{\tilde{x}}^2 (1+\varepsilon)C_{\varepsilon} }{\kappa_{2n}^2(s,
     3+4/\varepsilon)},
}
where $C_x=\sum_j \max_{i\ell}x_{ij\ell}^2$.
\end{corollary}

Persistency.

\begin{proposition}\label{prop:persist}
$$
|L(\hat\beta) - L(\beta)| \leqslant C_x \sum_{\ell} \|\hat\beta_{\cdot\ell} - \beta_{\cdot\ell}\|_2^2 +  \sum_{\ell}b_\ell\|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2,
$$
where $C_x=\sum_j \max_{i\ell}x_{ij\ell}^2$, $b_\ell =
2\sqrt{\sum_i c_{i\ell}^2}+1 $.
\end{proposition}
May be there is a sharper inequality?

\begin{proof} of Theorem~\ref{prop:persist}.

\begin{eqnarray*}
 |L(\hat\beta) - L(\beta)| &=& \left| \sum_{i,j}  (Y_{ij} - x_{ij\cdot}\t \hat\beta_i)^2  + \sum_{\ell} ||\hat\gamma_{\cdot \ell} ||_2     - \sum_{i,j}  (Y_{ij} - x_{ij\cdot}\t \beta_i)^2 -\sum_{\ell} ||\gamma_{\cdot \ell} ||_2   \right| \\
 &=& \left| \sum_{i,j} [  x_{ij\cdot}\t (\hat\beta_{i\cdot} + \beta_{i\cdot})  x_{ij\cdot}\t (\hat\beta_{i\cdot} - \beta_{i\cdot}) -2 Y_{ij} x_{ij\cdot}\t (\beta_i - \hat\beta_i)] + \sum_{\ell} ||\tilde\gamma_{\cdot \ell}-\gamma_{\cdot \ell} ||_2   \right| \\
 &=& \left| \sum_{i,j} x_{ij\cdot}\t (\hat\beta_{i\cdot} - \beta_{i\cdot}) [x_{ij\cdot}\t (\hat\beta_{i\cdot} + \beta_{i\cdot})  -2 (x_{ij\cdot}\t \beta_i +\varepsilon_{ij} )] + \sum_{\ell} ||\tilde\gamma_{\cdot \ell}-\gamma_{\cdot \ell} ||_2   \right| \\
 &=& \left| \sum_{i,j} x_{ij\cdot}\t (\hat\beta_{i\cdot} - \beta_{i\cdot}) [x_{ij\cdot}\t (\hat\beta_{i\cdot} - \beta_{i\cdot})  -2 \varepsilon_{ij} ] + \sum_{\ell} ||\tilde\gamma_{\cdot \ell}-\gamma_{\cdot \ell} ||_2 \right| \\
 &\leqslant& \sum_{i,j} [x_{ij\cdot}\t (\hat\beta_{i\cdot} - \beta_{i\cdot})]^2 +  2 \sum_{i,j} \left|x_{ij\cdot}\t (\hat\beta_{i\cdot} - \beta_{i\cdot})  \varepsilon_{ij} \right|  + \sum_{\ell} ||\tilde\gamma_{\cdot \ell}-\gamma_{\cdot \ell} ||_2 \\
 &\leqslant& \sum_{i,j} [x_{ij\cdot}\t (\hat\beta_{i\cdot} - \beta_{i\cdot})]^2 +  2\sum_{i\ell}c_{il}|\beta_{il}-\hat\beta_{i\ell}| + \sum_{\ell} ||\hat\beta_{\cdot \ell}-\beta_{\cdot \ell}
 ||_2\\
 &\leqslant& \sum_j \max_{i\ell}x_{ij\ell}^2 \sum_{i} \|\hat\beta_{i\cdot} - \beta_{i\cdot}\|_2^2 +  2\sum_{\ell}\sqrt{\sum_i c_{i\ell}^2}\|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2 + \sum_{\ell} ||\hat\beta_{\cdot \ell}-\beta_{\cdot \ell} ||_2\\
 &\leqslant&  \sum_j \max_{i\ell}x_{ij\ell}^2 \sum_{\ell} \|\hat\beta_{\cdot\ell} - \beta_{\cdot\ell}\|_2^2 +  \sum_{\ell}\left[2\sqrt{\sum_i c_{i\ell}^2}+1\right]\|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2,
\end{eqnarray*}
where the last 4 inequalities hold on event $\sca$ defined in the
proof of Lemma~\ref{lem:RotateGroupLasso}.

\end{proof}



==> SEBAsecSpectralTMP2.tex <==

\section{The spectral penalty}
\label{sec:spectral}


Let \(A=\sum c_i x_ix_i\t\), be a positive semi-definite matrix,
where \(x_1,x_2,\dots\) is an orthonormal basis of eigenvectors.
Then, we define \(A^{\gamma}=\sum c_i^{\gamma} x_ix_i\t\). We
consider now as penalty the function
 \eqsplit{
    \psi(\scb)=\psi(\beta_1,\dots,\beta_n)= \trace\Bigl\{\bigl(\summ i1n \beta_i\beta_i\t\bigr)^{1/2}\Bigr\}.
  }  Note that \(\psi(\scb)=\sum c_i^{1/2}\) where \(c_1,\dots,c_p\)  are the eigenvalues of \(\scb\scb\t=\summ i1n \beta_i\beta_i\t\) (including multiplicities).

\begin{lemma}
\label{lem:psiConvex}

\(\psi\) is a convex function.
\end{lemma}

In this section we study the estimator defined by
 \eqsplit[specPen]{
    (\hat\beta_1,\dots,\hat\beta_n)&= \argmin_{(\beta_1,\dots,\beta_n)\in\R^{p\times n}}\{\summ i1n (y_{ij}-x_{ij}\t\beta_i)^2+\lm\psi(\beta_1,\dots,\beta_n)\}
  }

The lassoes penalty considered primary the columns of \scb.  The
main focus of the group lasso was the rows. The spectral penalty
is symmetric in its treatment of the rows and columns since
$\spect\scb =\spect\scb\t$, where $\spect A$ denotes the spectrum
of $A$. Moreover, the penalty is invariant to the rotation of the
matrix \scb. In fact, \(\psi(\scb) = \psi(T\scb U )\), where \(T\)
and \(U\) are \(n\times n\) and \(p\times p\) rotation matrices:
 \eqsplit{
    (T\scb U)\t (T\scb U) &= U\t\scb\t\scb U
  }
and the RHS have the same eigenvalues as \(\scb\t\scb=\sum \beta_i\beta_i\t\).

Now, the standard notion  of sparsity, as captured by the $L_0$
norm, or by the standard lasso and group lasso, is basis
dependent. Consider the nonparametric setup in which $y_{ij} =
g(z_{ij}) + \eps_{ij}$, where $z\in[0,1]$. The model fits the
regression setup, if $x_{ij\ell}=h_\ell(z_{ij}$. If, for example,
$g(z)=\ind(a<z\le b)$, then this example is sparse when
$h_\ell(z)=\ind(z>\ell/p)$. It is not sparse if
$h_\ell(z)=(z-\ell/p)^+$. On the other hand a function $g$ which
has a piece-wise constant slope is sparse in the latter basis, but
not in the former.



The spectral penalty aims at finding a basis in which
$\beta_1,\dots,\beta_n$ have the same pattern of sparsity. This is
meaningless if $n$ is small --- any function is sparse in some
basis. However, we will argue that this can be done when $n$ is
large.


The following lemma describes a relationship between the group lasso and the spectral norm.

\begin{lemma}
\label{lem:spectVsGroup}
\mbox{}\par

\begin{enumerate}[(i)]
\item
$\|\scb\|_{2,1} \ge \inf_{U\in\scu} \|\scb\|_{2,1} =\psi(\scb)$, where $\scu$ is the set of all unitary matrices.
\item
There is a unitary matrix $U$, which may depend on the data, such that if $X_1,\dots,X_n$ are rotated by $U\t$, then the solution of the spectral penalty target function \eqref{specPen} is the solution of the group lasso in this basis.
\end{enumerate}

\end{lemma}

\subsection{The spectral penalty: 2D case}

In the 2-dimensional case ($p=2$), we can find the explicit
expression for the penalty in terms of $\beta_{\cdot \ell}$. The
eigenvalues of
 \eqsplit{
     \scb \scb\t = \begin{pmatrix}  ||\beta_{\cdot 1}||_2^2 & \langle \beta_{\cdot 1}, \beta_{\cdot 2}\rangle  \\ \langle \beta_{\cdot 1}, \beta_{\cdot 2}\rangle & ||\beta_{\cdot 2}||_2^2 \end{pmatrix}
%    &= \sigma\begin{pmatrix} \sum_i \ti\beta_i\ti\beta_i\t &  0 \\ 0 & t^2\sum b_i^2 - t^2\sum_i b_i\ti\beta_i\t \Bigl(\sum_i \ti\beta_i\ti\beta_i\t\Bigr)^{-1} \sum_ib_i\ti\beta_i \end{pmatrix} \\
%    &= \sig\Bigl(\sum \ti\beta_i\ti\beta_i\t\Bigr) \union t^2 \bigl(\sum b_i^2 - \sum_i b_i\ti\beta_i\t \Bigl(\sum_i \ti\beta_i\ti\beta_i\t\Bigr)^{-1} \sum_ib_i\ti\beta_i \bigr)
  }
are the solutions of $(||\beta_{\cdot 1}||_2^2 - z)(||\beta_{\cdot
2}||_2^2 - z) - \langle \beta_{\cdot 1}, \beta_{\cdot
2}\rangle^2=0$, i.e. are
$$
z_{1,2} = \frac 1 2 \left[ ||\beta_{\cdot 1}||_2^2 +
||\beta_{\cdot 2}||_2^2 \pm \sqrt{ \left(||\beta_{\cdot 1}||_2^2 -
||\beta_{\cdot 2}||_2^2\right)^2 + 4 \langle \beta_{\cdot 1},
\beta_{\cdot 2}\rangle^2} \right],
$$
and hence it can be shown that
$$
\psi(\scb) =z_1^{1/2}+ z_2^{1/2} = \sqrt{||\beta_{\cdot 1}||_2^2 +
||\beta_{\cdot 2}||_2^2 + 2 \sqrt{||\beta_{\cdot 1}||_2^2
||\beta_{\cdot 2}||_2^2 - \langle \beta_{\cdot 1}, \beta_{\cdot
2}\rangle^2}}
$$
due to identity $\sqrt{A + \sqrt{A^2-4B}} + \sqrt{A -
\sqrt{A^2-4B}} = \sqrt{2A +4\sqrt{B}}$.

Hence, in the directions where $\beta_{\cdot 1}$ and $\beta_{\cdot
2}$ are orthogonal, $\psi(\scb)$ behaves like $\ell_1$ penalty,
and in the directions they are collinear ($\langle \beta_{\cdot
1}, \beta_{\cdot 2}\rangle = \pm 1$) $\psi(\scb)$ behaves like
$\ell_2$ penalty.

The penalty ``ball'' (i.e., the curve $\psi=1$ in the $||\beta_{\cdot 1}||_2$
and $||\beta_{\cdot 2}||_2$ plane) is plotted in Figure \ref{figBall} for different values of $\rho=\frac{\langle \beta_{\cdot 1}, \beta_{\cdot
2}\rangle}{||\beta_{\cdot 1}||_2 ||\beta_{\cdot 2}||_2}$,  the ``correlation'' between $\beta_{\cdot 1}$ and $\beta_{\cdot
2}$.

%\begin{figures}
\onefigure[0.7]{SpectBall.eps}{ The spectral ``ball'' in the $ ||\beta_{\cdot 1}||_2$ and $||\beta_{\cdot 2}||_2$ plane for
different values of $\rho$. }{figBall}
%\end{figures}

\subsection{The estimator  }

Let $\scb=\summ \xi1{p\wedge n}\al_\xi \beta_\xi^*{\be_\xi^*}\t$
be the spectral value decomposition,  or the PCA, of \scb:
$\beta_1^*,\dots,\beta_p^*$ and $\be_1^*,\dots,\be_n^*$ are
orthonormal sub-bases  of $\R^p$ and $\R^n$ respectively,
$\al_1\geq\al_2\geq\dots$, and
$\scb\scb\t\beta_\xi^*=\al_\xi^2\beta_\xi^*$,
$\scb\t\scb\be_\xi^*=\al_\xi^2\be_\xi^*$, $\xi=1,\dots,p\wedge n$.
%NB
Let $T=\summ \xi1{p\wedge n} e_\xi{\beta_\xi^*}\t$ (clearly,
$TT\t=I$).
% end NB
Consider the parametrization of the problem in the  rotated
coordinates, $\ti x_{ij}=Tx_{ij}$ and  $\ti\beta_i=T\beta_i$. Then
geometrically the regression problem is invariant:
$x_{ij}\t\beta_i=\ti x_{ik}\t\ti\beta_i$, and
$\psi(\scb)=\|\ti\scb\|_{2,1} $,
%NB
up to a modified regression matrix.
%NB

The  representation $\hat\scb = \summ \xi1s \al_\xi \beta_\xi^*
{\be_\xi^*}\t$ shows that the difficulty of the problem is the
difficulty of estimating $s(n+p)$ parameters with $nm$
observations. Thus it is feasible as long as $s/m\to0$ and $sp/nm\to0$

 We have

\begin{theorem}
\label{th:sparseSpect}
Suppose $p<n$. Then the solution of the least squares with the spectral penalty is given by $\summ \xi1s \beta^*_\xi{\be_\xi^*}\t$, $s=s_\lm \leq p$, and $s_\lm\dec 0$ as $\lm\to\en$. If $s=p$ then the gradient of the target function is given in a matrix form by
 \eqsplit{
    -2R+\lm (\hat\scb\hat\scb\t)^{-1/2}\hat\scb
  }
where
 \eqsplit{
    R=\Bigl(X_1\t(Y_1-X_1\hat\beta_1),\dots,X_n\t(Y_n-X_n\hat\beta_n)\Bigr).
  }
And hence
 \eqsplit{
    \hat\beta_i=\bigl(  X_i\t X_i + \frac\lm2 (\hat\scb\hat\scb\t)^{-1/2}\bigr)^{-1}X_i\t Y_i.
  }
That is, the solution of a ridge regression with adaptive weight.


More  generally, let $\hat\scb=\summ \xi1s \alpha_\xi
\beta_\xi^*{\be_\xi}\t$, $s<p$, where $\beta_1^*,\dots,\beta_p^*$
is an orthonormal base of $\R^p$. Then the solution satisfies
 \eqsplit{
    &{\beta_\xi^*}\t R = \frac\lm2 {\beta_\xi^*}\t   (\hat\scb\hat\scb\t)^{+1/2}\hat\scb, \quad \xi\leq s
    \\
    &|{\beta_\xi^*}\t R \be_\xi^*| \leq \frac\lm 2,  \qquad \qquad \qquad s<\xi\leq p.
  }
where for any positive semi-definite matrix $A$, $A^{+1/2}$ is the Moore-Penrose  generalized inverse of $A^{1/2}$.
\end{theorem}
Roughly speaking the following can be concluded from the  theorem.
Suppose the data were generated by a sparse model (in \emph{some}
basis). Consider the problem in the transformed basis, and let $S$
be the set of non-zero coefficients of the true model. Suppose
that the design matrix is of full rank within the sparse model:
$X_i\t X_i=\O(m)$, and  that \lm is chosen such that $\lm\gg
\sqrt{nm\log(np)}$.  Then the coefficients corresponding to $S$
satisfy
 \eqsplit{
   \hat\beta_{Si} &= \bigl(X_i\t X_i + \frac\lm2 (\hat\scb_S\hat\scb_S\t)^{1/2}\bigr)^{-1}X_i\t Y_i.
  }
 Since it is expected that  $\lm(\scb_S\scb_S\t)^{1/2}$ is only slightly larger than $\O(m\log(np))$, it is completely dominated
  by $X_i\t X_i$, and the estimator of this part of the model is consistent. On the other hand, the rows of $R$ corresponding
  to coefficient not in the true model are only due to noise and hence each of them is  $\O(\sqrt {nm})$.
  The factor of $\log (np)$ ensures that their maximal norm will be below $\lm/2$, and the estimator is consistent.

\subsection{Bayesian perspectives}

We consider now the penalty for $\beta_k$ for a fixed $k$. Let $A=n^{-1}\sum_{k\ne i} \beta_k\beta_k\t$.  Using Taylor expansion for not too big $\beta_i$,  based on \eqref{eigender} we get
\eqsplit{
    \trace\bigl( (nA+\beta_i\beta_i\t)^{1/2}\bigr)
     &= \sqrt{n}\trace(A^{1/2}) + \summ j1p \frac{x_j\t \beta_i\beta_i\t x_j}{2 c_j^{1/2}}
     \\
    &= \sqrt{n}\trace(A^{1/2}) + \frac 12 \beta_i\t \bigl(\sum c_j^{-1/2} x_jx_j\t\bigr)\beta_i
    \\
    &= \sqrt{n}\trace(A^{1/2}) + \frac12 \beta_i\t A^{-1/2}\beta_i
}
So, this like $\beta_i$ has a prior of $\normal(0, n \sig^2/\lm A^{1/2})$. Note that the prior is only related to the estimated variance of $\beta$, and $A$ appears with the power of $1/2$. Now $A$ is not really the estimated variance of $\beta$, only the variance of the estimates, hence it should be inflated, and the square root takes care of that. Finally, note that eventually, if $\beta_i$ is very large relative to $nA$, then the penalty become $\|\beta\|$, so the ``prior'' becomes essentially normal, but with exponential tails.

A  better way to look on the penalty from a Bayesian perspective is to consider it as prior on the \(n\times p\) matrix \(\scb=(\beta_1,\dots,\beta_n)\). Recall that the penalty is invariant to the rotation of the matrix \scb. In fact, \(\psi(\scb) = \psi(T\scb U )\), where \(T\) and \(U\) are \(n\times n\) and \(p\times p\) rotation matrices. Now, this means that if \(\be_1,\dots,\be_p\) are orthonormal set of eigenvectors of \(\scb\t\scb\) and \(\gamma_{ij}=\be_j\t\beta_i\) --- the PCA of \(\beta_1,\dots,\beta_n\), then \(\psi(\scb) = \summ j1p \bigl(\summ i1n \gamma_{ij}^2\bigr)^{1/2} \) --- the rms penalty in terms of the principal components. The ``prior'' is then proportional to $ e^{-\lm \summ j1p \|\gamma_{\cdot j}\|_2}$.\, which is as if to obtain a random $\scb$ from the prior the following procedure should be followed:

\begin{enumerate}%[(i)]
\item
Sample \(r_1,\dots,r_p\) independently from \(\Gamma(n,\lm)\) distribution.
\item
For each \(j=1,\dots,p\) sample \(\gamma_{1j},\dots,\gamma_{nj}\) independently and uniformly on the sphere with radius \(r_j\).
\item
Sample an orthonormal base \(\chi_1,\dots,\chi_p\) "uniformly''.
\item
Construct \(\beta_i = \summ j1p \gamma_{ik}\chi_k\).
\end{enumerate}
So hopefully the rms penalty ensures that the solution will be sparse in \emph{some} basis. It works when the assumption (and hope) is that the Procrustes's distance between the true \(\beta\)'s and a sparse solution is small.

\subsection{Algorithm and small simulation study}

%\begin{figures}
\twofigures[1.1]{NB03042009a.eps}{NB03042009b.eps}{Component
variances and eigenvalues, \(m=25\), \(n=150\) }{fig1}
%\end{figures}

A simple algorithm is the following:
\begin{enumerate}%[(i)]
\item Initiate some small value of \(\hat
\beta_1,\dots,\hat\beta_n\). Let \(A=\summ j1n
\hat\beta_j\hat\beta_j\t\). Fix  \(\gamma\in(0,1]\), \(\eps>0\),
\(k\), and \(c>1\). \item\label{A1st1} For \(i=1,\dots,n\):
\begin{enumerate}%[(i)]
\item Compute \(\delta_i = (X_i\t X_i + \lm A^{-1/2})^{-1}X_i\t
(y_i-X_i\hat\beta_i)\). \item Update \(A\leftarrow
A-\hat\beta_i\hat\beta_i\);
\(\hat\beta_i\leftarrow\hat\beta_i+\gamma\delta_i\); \(A\leftarrow
A+\hat\beta_i\hat\beta_i\);
\end{enumerate}
\item if \(\summ j1p \ind\bigl(n^{-1}\summ
i1n\hat\beta_{ij}^2>\eps\bigr)>k \) update
\(\lambda\leftarrow\lambda c\) otherwise
\(\lambda\leftarrow\lambda/ c\). \item Return to step \ref{A1st1}
unless there is no real change of coefficients.
\end{enumerate}

Comment: to fasten the computation, the SVD was computed only
every 10 values of \(i\).

As a simulation we applied the above algorithm to the following
simulated data.
%  (\textbf{NB05Apr2009.m})..
We generated random \(\beta_1,\dots,\beta_{150}\in\R^{150}\) such that all coordinates
are independent, and \(\beta_{ij}\dist\normal(0, e^{-2j/5})\). All
\(X_{ij\ell}\) are \iid \(\normal(0,1)\), and \(y_{ij} =
x_{ij\cdot}\t \beta_i+\eps_{ij}\), where \(\eps_{ij}\) are all
\iid \(\normal(0,1)\).  The true \(R^2\) obtained was
approximately  0.73. The number of replicates per value of
\(\beta\), \(m\), varied between 5 to 300. We consider two
measures of estimation error:
 \eqsplit{
    L_{\rm par} &= \frac{\summ i1n \|\hat\beta_i-\beta_i\|_\en} {\summ i1n \|\beta_i\|_\en}
    \\
    L_{\rm pre}  &= \frac{\summ i1n \|X_j(\hat\beta_i-\beta_i)\|_\en} {\summ i1n \|X_i\beta_i\|_\en}
  }


%\begin{figures}
\onefigure[1.1]{NB11Apr2009d.eps}{ Lower lip position while
repeating 32 times 'Say bob again'}{fig2}
%\end{figures}

The algorithm stopped after 30--50 iterations. Figure \label{fig1}
is a graphical presentation of a typical result. A summary is
given in Table \ref{tab1}. Note that \(m\) has a critical  impact
on the estimation problem. However, with as little as \(5\)
observations per \(R^{150}\) vector of parameter we obtain a
significant reduction in the prediction error.
\begin{table}[H]
\caption{\label{tab1}The estimation and prediction error as
function of the number of observations per vector of parameters
Means (and SDK).}
\begin{center}

\begin{tabular}{|r|r|r|}
\hline
$m$     &   \(L_{\rm par}\)  & $L_{\rm pre}$    \\
\hline\hline
5  &    0.9530 (0.0075)               &   0.7349 (0.0375)         \\
\hline
25  &   0.7085 (0.0289)                &  0.7364 (0.0238)           \\
\hline
300  &  0.2470 (0.0080)                 &  0.5207 (0.0179)          \\
\hline

\end{tabular}
\end{center}
\end{table}


%\begin{figures}
\threefiguresV[1.5]{NB11Apr2009a.eps}{NB11Apr2009b.eps}{NB11Apr2009c.eps}{Eigenvalue,
coefficient variance and typical observed and smooth path.}{fig3}
%\end{figures}

The technique is natural for functional data analysis. We used the
data LipPos. The data is   described by %James O.
Ramsay and
%Bernard W.
Silverman and can be found in
http://www.stats.ox.ac.uk/~silverma/fdacasebook/lipemg.html. The
original data is given in Figure \ref{fig2}. However we added noise to
the data as can be seen in Figure \ref{fig3}. The lip position is
measured at $m=501$ time points, with \(n=32\) repetitions.


As the matrix \(X\) we considered the union of 6 cubic spline
bases with, respectively, 5, 10, 20, 100, 200, and 500 knots
(i.e., \(p=841\), and \(X_i\) does not depend on \(i\)). A
Gaussian noise with \(\sigma=0.001\) was added to \(Y\). The
result of the analysis is given in Figure \ref{fig3}. Figure
\ref{fig4} present the projection of the mean path on the first
eigen-vectors of \(\summ i1n \hat\beta_i\hat\beta_i\t\).
%(Analysis done using NB11Apr2009.m).


%\begin{figures}
\onefigure[0.5]{NB11Apr2009e.eps}{Projection of the estimated mean
path on the 2 first eigen-vectors of \(\summ i1n
\hat\beta_i\hat\beta_i\t\) and the true mean path.}{fig4}
%\end{figures}

The final example we consider is some what arbitrary. The data,
taken from StatLib, is of the daily wind speeds for 1961-1978 at
12 synoptic meteorological stations in the Republic of Ireland. As
the \(Y\) variable we considered one of the stations (station
BIR). As explanatory variables we considered the 11 other station
of the same day, plus all 12 stations 70 days back (with the
constant we have altogether 852 explanatory variables). The
analysis was stratified by month. For simplicity, only the first
28 days of the month were taken, and the first year, 1961, served
only for explanatory purpose. The last year was served only for
testing purpose, so, the training set was for 16 years (\(N=12\),
\(m=448\), and \(P=852\) ).  In Figure \ref{fig5} we give the 2nd
moments of the coefficients and the scatter plot of predictions
vs. true value of the last year.
%(Analysis done using NB14Apr2009.m)

%\begin{figures}
\twofigures[0.75]{NB14Apr2009a.eps}{NB14Apr2009b.eps}{Coefficient
2nd moment and prediction vs.true value of the test year.}{fig5}
%\end{figures}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{The spectral penalty: oracle inequalities}

%[assumption: $X_{i\cdot \ell}X_{i\cdot \ell}\t =C$, for all $i$ and $\ell$. ]

If $\beta\beta\t = U C U\t$ and $\hat\beta\hat\beta\t = \hat{U}
\hat{C} \hat{U}\t$ where $\hat\beta$ is the solution of the
spectral RMS problem \eqref{rotatedlassostar}. Then $U\t\hat\beta$
is the solution of the standard group lasso problem
\eqref{lassostar} with $\tilde{X}_i = U^T X_i$. Hence,
Lemma~\ref{lem:GroupLasso} is satisfied for $\gamma = U\t\beta$
and ``estimate'' $\tilde\gamma = U\t\hat\beta$ with design
matrix $\tilde{X}$.

Note that even if $\beta$ and $\hat\beta$ are close, $\gamma$ and
$\hat\gamma = \hat{U}\t\hat\beta$ are close only up to a
permutation of variables. Hence, we will be interested in
comparing $U\t\hat{U}$ to a permutation matrix (e.g. testing that
 all eigenvalues are close to $\pm 1$).

We may be interested in sparsity of $\beta$ and $\gamma$, as well
as the approximation error of estimating $f$ and $\beta$. Thus, we
obtain the following results.




\begin{lemma}\label{lem:RotateGroupLasso}
Let \(y_{ij}\dist \normal (f_{ij},\sig^2)\) independent,
\(f_{ij}=x_{ij}\t\beta_i\), \(x_{ij}\in \R^p\),
\(\beta_i\in\R^p\), \(i=1,\dots,n\), \(j=1,\dots,m\).  Consider
 \eqsplit[rotatedlassostar]{
    (\hat\beta_1,\dots,\hat\beta_n) &=
    \argmin \Biggl[ \summ i1n \summ j1m (y_{ij} - x_{ij}\t\,\beta_i)^2 + \lambda
   \trace  \Bigl\{ \summ i1n \beta_{i }\beta_i^T\Bigr\}^{1/2}
   \Biggr].
  }
Assume that $\summ j1m x_{ij\ell}^2 = m$ for all $i, \, \ell$.

Fix some $c>0$ (which may depend on $p$, $n$ and $m$), and take
$\lambda = 4 \sigma\sqrt{m  (p + c)}$. Then, with probability at
least \(
 1-\exp\left( -\frac n 8 \min(c, c^2/p) \right)\):
\begin{enumerate}[a)]

\item \(\forall \beta\in\R^{p\times n}\):%
  \eqsplit[SPECTboundf_beta1]{ %
 &\hspace{-3em}\|f_{\beta}-\hat f\|_2^2 + \frac{\lambda} 2 \sum_{\ell} ||(U\t\hat{U} \hat\gamma)_{\cdot
 \ell} -  \gamma_{\cdot \ell}||_2 
 \\ &  \leqslant  2\lambda \sum_{\ell \in J(\gamma)}
\|\gamma_{\cdot \ell}- (U\t\hat{U} \hat\gamma)_{\cdot
 \ell}\|_2 + \lambda
\sum_{\ell} (\| (U\t\hat{U} \hat\gamma)_{\cdot
 \ell}\|_2 - \|\hat\gamma_{\cdot \ell}\|_2),
  }
where \(f_{\scb ij} = x_{ij}\t\beta_i = x_{ij}\t U\t \gamma_i \),
%$\lambda = 4\sqrt{n}\max_i \sqrt{\sum_j c_{ij}^2}$
 and%
 \eqsplit{
J(\gamma)=\Bigl\{\ell\in\{1,\dots,p\}:\summ i1n\gamma_{i\ell}^2>0\Bigr\}. %
 }

\item $\scm(\hat\gamma)\leqslant \frac{\phi^2_{\max} (X\t
X/m)}{\kappa^2} \, s$ \,\, [under restricted e.v. assumption - to
be moved to the theorem].

 \item   $||U  - \hat{U} ||_2 \leqslant 2 C_{\beta, \hat\beta}
\sum_i ||\hat\beta_i - \beta_i||_2 \left(||\beta_i||_2 + \sum_i
||\hat\beta_i - \beta_i||_2 \right)$,

where $C_{\beta, \hat\beta}^2 = \sum_k \sup_{t\in(0,1)} \max_{j:
\,  j\neq  k} \frac 1 {(c_j(t) - c_k(t))^2}$,

 $c_k(t)$ are the eigenvalues of \( A(t)=\summ i1n
\bigl( (1-t)\beta_i + t\hat\beta_i  \bigr)\bigl((1-t)\beta_i +
t\hat\beta_i\bigr)\t\).

Hence, the rotations $U$ and $\hat{U} $ are close if \scb has
distinct eigen values.

\end{enumerate}
\end{lemma}

[up to here]

We need one of the following assumptions. Following (e.g.
Obozinski et al, 2008), denote $||x||_{p/q} = \summ i1n \left[||
x_{\cdot i} ||_p^q \right]^{1/q}$, $x\in \mathbb{R}^{m\times n}$.

\noindent{\bf Assumption URE2$_n(s; c_0)$}. For some integer $s$ such that
$1 \leqslant s \leqslant p$, and a positive number $c_0$ the
following condition holds:
\begin{equation}
\tilde{\kappa}_{U \, n}(s, c_0)^2 := \min_i \min_{\substack{J_0
\subseteq \{1,\dots,\,p\},\\ |J_0|\leqslant\, s}} \,
\min_{U\in \mathbb{R}^{p\times p}: \, U U\t = I} \min_{\substack{\delta \in \mathbb{R}^{n\times p}\setminus \{0\}, \\
 ||\delta_{ \cdot \, J_0^c}||_{2/1} \leqslant \, c_0
 ||\delta_{ \cdot \, J_0}||_{2/1}  }} \frac{|| X_{i\cdot\cdot}^T U \delta_i||_2^2}{|| \delta_{i J_0}||_2^2} > 0.
\end{equation}


\noindent{\bf Assumption MURE2$_n(s; c_0)$}. For some integer $s$ such that
$1 \leqslant s \leqslant p$, and a positive number $c_0$ the
following condition holds:
\begin{equation}
\tilde{\kappa}_{U \, n}(s, c_0)^2 := \min_{\substack{J_0 \subseteq
\{1,\dots,\,p\},\\ |J_0|\leqslant\, s}} \,
\min_{U\in \mathbb{R}^{p\times p}: \, U U\t = I} \min_{\substack{\delta \in \mathbb{R}^{n\times p}\setminus \{0\}, \\
 ||\delta_{ \cdot \, J_0^c}||_{2/1} \leqslant \, c_0
 ||\delta_{ \cdot \, J_0}||_{2/1}  }} \frac{\summ i1n ||
X_{i\cdot\cdot}^T U \delta_i||_2^2}{ \summ i1n || \delta_{i
J_0}||_2^2} > 0.
\end{equation}

% analogue of Theorem 6.1 in BRT
\begin{theorem}
\label{th:BRTspectral}

 Let \(y_{ij}\dist \normal (f_{ij},\sig^2)\) independent,
\(f_{ij}=x_{ij}\t\beta_i\), \(x_{ij}\in \R^p\),
\(\beta_i\in\R^p\), \(i=1,\dots,n\), \(j=1,\dots,m\), $p\geqslant
2$.  Fix some $\varepsilon  > 0$ and let Assumption MURE2$_n(s; 3
+ 4/\varepsilon)$ (or Assumption URE2$_n(s; 3 + 4/\varepsilon)$)
be satisfied for $X=(x_{ijl})$.

Consider the spectral RMS estimator $\hat{f}_{ij} =
X_{ij}\t\hat{\beta}_i$ where $\hat{\beta}$ is defined by
\eqref{rotatedlassostar} with \(\lm=4A\sig\tilde\Lm_x\sqrt{n
\log(pn)}\), where \(\tilde\Lm_x= \max_{i}\sqrt{\sum_{\ell,j} x_{i
j \ell}^2 }\) and \(A>\sqrt2\).

Then, with probability at least \(1-(np)^{1-A^2/2}\),
   \eqsplit{ %
     \|f-\hat f\|_2^2  \le (1+\varepsilon)\inf_{\substack{\beta\in\mathbb{R}^p,\\ \scm(\gamma)\le s}} \left[\|f - f_{\scb}\|_2^2
     + \scm(\gamma) n\log(np) \frac{16 A^2 \sigma^2
     \Lambda_{\tilde{x}}^2 C_{\varepsilon} }{\kappa_{2n}^2(s, 3+4/\varepsilon))}\right],
     } %
where  $C_{\varepsilon} = \frac{(\varepsilon+2)^2}{\varepsilon
(1+\varepsilon)} >0$.

Also, we can show that
   \eqsplit{ %
     \|f-\hat f\|_2  \le (1+\varepsilon) \inf_{\substack{\beta\in\mathbb{R}^p,\\ \scm(\gamma)\le s}} \left[\|f - f_{\scb}\|_2
     + 2\lambda \frac{\sqrt{\scm(\gamma)} }{\kappa (s,
     3+4/\varepsilon) )}\right].
     } %

\end{theorem}


For linear regression, we obtain the following inequalities.
\begin{corollary}
\eqsplit{
 \frac 1 n \sum_{i=1}^n ||X_i\t(\beta_i -
\hat\beta_{i})||_2^2 &\leqslant \scm(\gamma) \log(np) \frac{16 A^2
\sigma^2
     \Lambda_{\tilde{x}}^2 C_{\varepsilon} }{\kappa_{2n}^2(s,
     3+4/\varepsilon)},\\
\frac 1 n \sum_{i=1}^n ||\beta_i - \hat\beta_{i}||_2^2 &\leqslant
C_x \scm(\gamma) \log(np) \frac{16 A^2 \sigma^2
     \Lambda_{\tilde{x}}^2 (1+\varepsilon)C_{\varepsilon} }{\kappa_{2n}^2(s,
     3+4/\varepsilon)},
}
where $C_x=\sum_j \max_{i\ell}x_{ij\ell}^2$.
\end{corollary}

Persistency.

\begin{proposition}\label{prop:persist}
$$
|L(\hat\beta) - L(\beta)| \leqslant C_x \sum_{\ell} \|\hat\beta_{\cdot\ell} - \beta_{\cdot\ell}\|_2^2 +  \sum_{\ell}b_\ell\|\beta_{\cdot\ell}-\hat\beta_{\cdot\ell}\|_2,
$$
where $C_x=\sum_j \max_{i\ell}x_{ij\ell}^2$, $b_\ell =
2\sqrt{\sum_i c_{i\ell}^2}+1 $.
\end{proposition}
May be there is a sharper inequality?

